Unconventional Materials: the mismatch between electronic charge centers and atomic positions

The complete band representations (BRs) have been constructed in the work of topological quantum chemistry. Each BR is expressed by either a localized orbital at a Wyckoff site in real space, or by a set of irreducible representations in momentum space. In this work, we define unconventional materials with a common feature of the mismatch between average electronic centers and atomic positions. They can be effectively diagnosed as whose occupied bands can be expressed as a sum of elementary BRs (eBRs), but not a sum of atomic-orbital-induced BRs (aBRs). The existence of an essential BR at an empty site is described by nonzero real-space invariants (RSIs). The "valence" states can be derived by the aBR decomposition, and unconventional materials are supposed to have an uncompensated total "valence" state. The high-throughput screening for unconventional materials has been performed through the first-principles calculations. We have discovered 423 unconventional compounds, including thermoelectronic materials, higher-order topological insulators, electrides, hydrogen storage materials, hydrogen evolution reaction electrocatalysts, electrodes, and superconductors. The diversity of these interesting properties and applications would be widely studied in the future.

==> table.tex <==
\begin{longtable}[!h]{|c|c|c|c|c|c|c|p{2cm}<{\centering}|p{1.5cm}|p{1cm}|c|}
\caption{The results of unconventional materials}
\\ \hline
 ICSD & Formula & NoA & NoE & E$_{g}$(eV) & E$_{ind}$(eV) & SG & Wyckoff positions & Length of bonds & Center & The essential BR\\
\hline
\color{black}{ 24981} & \hyperref[subfig:24981]{GdO} & 2 & 15 &  0.522 &  0.257 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 191788} & \hyperref[subfig:191788]{MnP} & 2 & 12 &  0.035 & -0.069 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 236788} & \hyperref[subfig:236788]{MnN} & 2 & 12 &  0.443 &  0.120 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 191171} & \hyperref[subfig:191171]{MnSn} & 2 & 11 &  0.109 &  0.050 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 167875} & \hyperref[subfig:167875]{HfN} & 2 & 9 &  0.035 & -0.654 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 167876} & \hyperref[subfig:167876]{TaN} & 2 & 10 &  0.000 & -0.977 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 30334} & \hyperref[subfig:30334]{SiP} & 2 & 9 &  0.220 & -2.997 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 167870} & \hyperref[subfig:167870]{TcN} & 2 & 12 &  0.243 & -0.333 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 186876} & \hyperref[subfig:186876]{MoP} & 2 & 11 &  0.048 & -0.220 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 186243} & \hyperref[subfig:186243]{IrN} & 2 & 14 &  0.000 & -2.506 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 183192} & \hyperref[subfig:183192]{RhN} & 2 & 14 &  0.000 & -2.908 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 183190} & \hyperref[subfig:183190]{RuN} & 2 & 13 &  0.000 & -2.678 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 150682} & \hyperref[subfig:150682]{Cu} & 2 & 22 &  0.286 & -0.365 &  12 & 4g & &&Ag@2b\\
\hline
\color{black}{ 183184} & \hyperref[subfig:183184]{NbN} & 2 & 16 &  0.000 & -0.849 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 187182} & \hyperref[subfig:187182]{MoN} & 2 & 11 &  0.034 & -0.625 & 216 & 4d,4a & &&A1@4c\\
\hline
\color{black}{ 41258} & \hyperref[subfig:41258]{FeN} & 2 & 13 &  0.000 & -3.269 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 183182} & \hyperref[subfig:183182]{ZrN} & 2 & 17 &  0.000 & -0.671 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 181079} & \hyperref[subfig:181079]{CrN} & 2 & 11 &  0.341 & -0.016 & 216 & 4c,4a & &&A1@4b\\
\hline
\color{black}{ 167879} & \hyperref[subfig:167879]{OsN} & 2 & 13 &  0.352 & -1.858 & 216 & 4c,4a & &&A1@4d\\
\hline
\color{black}{ 22231} & \hyperref[subfig:22231]{Ca$_{2}$N} & 3 & 25 &  0.331 &  0.035 & 166 & 6c,3a & &&A1g@3b\\
\hline
\color{black}{ 67443} & \hyperref[subfig:67443]{NbS$_{2}$} & 3 & 23 &  1.641 &  1.316 & 187 & 1a,2i &  S:3.124 & S:1e  &A1'@1c\\
\hline
38245 & \hyperref[subfig:38245]{KO$_{2}$} & 3 & 21 &  4.349 &  3.858 & 139 & 4e,2b &  O:1.306 & O:2a  &A1g@2a\\
\hline
290427 & \hyperref[subfig:290427]{HfN$_{2}$} & 3 & 14 &  0.069 & -0.574 & 187 & 2h,1b &  N:1.441 & N:1c  &A1'@1c\\
\hline
48214 & \hyperref[subfig:48214]{HgO$_{2}$} & 3 & 24 &  1.265 &  0.348 &  12 & 2a,4i &  O:1.494 & O:2d  &Ag@2d\\
\hline
290430 & \hyperref[subfig:290430]{TaN$_{2}$} & 3 & 15 &  1.474 &  0.646 & 187 & 2g,1f &  N:1.399 & N:1a  &A1'@1d\&A1'@1a\\
\hline
\color{black}{ 54255} & \hyperref[subfig:54255]{MnNiSb} & 3 & 22 &  0.026 & -0.073 & 216 & 4c,4d,4a & &&A1@4b\\
\hline
251718 & \hyperref[subfig:251718]{CrSe$_{2}$} & 3 & 18 &  0.039 & -0.288 &  12 & 2a,4i & Se:3.488 &Se:2b  &Ag@4e\&Ag@2b\\
 & & & & & & & & & &Ag@4e\&Bg@2b\\
\hline
\color{black}{ 414330} & \hyperref[subfig:414330]{Sr$_{2}$N} & 3 & 25 &  0.246 & -0.134 & 166 & 6c,3a & &&A1g@3b\\
\hline
647338 & \hyperref[subfig:647338]{RbO$_{2}$} & 3 & 21 &  4.205 &  3.748 & 139 & 2a,4e &  O:1.332 & O:2b  &A1g@2b\\
\hline
\color{black}{ 58108} & \hyperref[subfig:58108]{Al$_{2}$Os} & 3 & 14 &  1.172 &  0.245 & 139 & 2a,4e & &&Ag@4c\\
\hline
\color{black}{ 54465} & \hyperref[subfig:54465]{MnSnAu} & 3 & 22 &  0.042 & -0.008 & 216 & 4c,4b,4a & &&A1@4d\\
\hline
\color{black}{ 187135} & \hyperref[subfig:187135]{LiFeP} & 3 & 14 &  0.459 & -0.061 & 107 & 2a & &&A@4b\\
\hline
\color{black}{ 51975} & \hyperref[subfig:51975]{Mg$_{3}$In} & 4 & 9 &  0.153 & -3.088 & 221 & 3c,1a & &&A1g@1b\\
\hline
\color{black}{ 57827} & \hyperref[subfig:57827]{TiAlFe$_{2}$} & 4 & 23 &  0.235 &  0.203 & 225 & 4b,8c,4a & &&Ag@24d\\
\hline
\color{black}{ 240110} & \hyperref[subfig:240110]{LiAl} & 4 & 8 &  0.462 & -0.494 & 227 & 8a,8b & &&A1g@16d\\
\hline
\color{black}{ 57832} & \hyperref[subfig:57832]{AlVFe$_{2}$} & 4 & 24 &  0.171 & -0.066 & 225 & 4b,8c,4a & &&Ag@24d\\
\hline
\color{black}{ 620612} & \hyperref[subfig:620612]{ZrCd} & 4 & 48 &  0.013 & -0.973 & 129 & 2c & &&A1@2b\&B1@2b\\
 & & & & & & & & & &A1@2a\&B1@2a\\
\hline
\color{black}{ 633766} & \hyperref[subfig:633766]{TiFe$_{2}$Sn} & 4 & 24 &  0.142 &  0.105 & 225 & 8c,4b,4a & &&Ag@24d\\
\hline
\color{black}{ 633246} & \hyperref[subfig:633246]{FeSiRu$_{2}$} & 4 & 28 &  0.108 & -0.217 & 225 & 4b,8c,4a & &&Ag@24d\\
\hline
\color{black}{ 35701} & \hyperref[subfig:35701]{ZrCl} & 4 & 38 &  0.045 & -0.620 & 164 & 2d & Cl:3.782 &Cl:3e  &A1g@1b\\
\hline
\color{black}{ 631850} & \hyperref[subfig:631850]{VGaFe$_{2}$} & 4 & 24 &  0.223 & -0.152 & 225 & 4b,8c,4a & &&Ag@24d\\
\hline
\color{black}{ 616286} & \hyperref[subfig:616286]{HfBe} & 4 & 12 &  0.020 & -1.993 &  63 & 4c & &&Ag@4b\\
\hline
\color{black}{ 249592} & \hyperref[subfig:249592]{SrMgIn$_{3}$} & 5 & 21 &  0.000 & -1.195 & 119 & 2d,2a,2c,4e & &&B1@2d\&A1@2b\\
 & & & & & & & & & &B1@2c\&A1@2b\\
\hline
\color{black}{ 43690} & \hyperref[subfig:43690]{Ge$_{2}$Os} & 6 & 32 &  0.299 & -0.168 &  12 & 4i & &&Ag@2c\&Ag@2a\\
\hline
\color{black}{ 163696} & \hyperref[subfig:163696]{YMgCu$_{4}$} & 6 & 57 &  0.150 & -0.893 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
\color{black}{ 58156} & \hyperref[subfig:58156]{Al$_{2}$Ru} & 6 & 28 &  1.227 &  0.129 &  70 & 8b,16f & &&Ag@16d\&A@8b\\
 & & & & & & & & & &Ag@16d\&A@8a\\
\hline
\color{black}{ 658914} & \hyperref[subfig:658914]{CaInCu$_{4}$} & 6 & 57 &  0.765 & -0.505 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
\color{black}{ 194977} & \hyperref[subfig:194977]{NdMgCu$_{4}$} & 6 & 57 &  0.008 & -0.887 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
\color{black}{ 616387} & \hyperref[subfig:616387]{Be$_{5}$Pd} & 6 & 20 &  0.334 & -0.644 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
\color{black}{ 416528} & \hyperref[subfig:416528]{ScInCu$_{4}$} & 6 & 50 &  0.435 & -0.350 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
\color{black}{ 156265} & \hyperref[subfig:156265]{HfGaAu} & 6 & 36 &  0.565 & -0.920 & 187 & 1a,2h,1b,2i & &&A1'@1e\&A1'@1d\\
 & & & & & & & & & &A1'@1e\&E''@1d\\
 & & & & & & & & & &E''@1e\&A1'@1d\\
 & & & & & & & & & &E''@1e\&E''@1d\\
\hline
\color{black}{ 156264} & \hyperref[subfig:156264]{ZrGaAu} & 6 & 52 &  0.473 & -0.766 & 187 & 1a,2h,1b,2i & &&A1'@1e\&A1'@1d\\
 & & & & & & & & & &A1'@1e\&E''@1d\\
 & & & & & & & & & &E''@1e\&A1'@1d\\
 & & & & & & & & & &E''@1e\&E''@1d\\
\hline
\color{black}{ 616395} & \hyperref[subfig:616395]{Be$_{5}$Pt} & 6 & 20 &  0.667 &  0.039 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
44751 & \hyperref[subfig:44751]{FeSe$_{2}$} & 6 & 40 &  0.954 &  0.356 &  58 & 4g,2a & Se:2.505 &Se:2c  &Ag@2c\\
\hline
\color{black}{ 103055} & \hyperref[subfig:103055]{MgCu$_{4}$Sn} & 6 & 50 &  0.126 & -1.443 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
\color{black}{ 186627} & \hyperref[subfig:186627]{FeSb$_{2}$} & 6 & 36 &  0.127 & -0.176 &  58 & 4g,2a & Sb:2.859 &Sb:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
\color{black}{ 628179} & \hyperref[subfig:628179]{YInCu$_{4}$} & 6 & 58 &  0.500 & -0.237 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
\color{black}{ 80945} & \hyperref[subfig:80945]{KSb$_{2}$} & 6 & 38 &  0.614 &  0.220 &  12 & 4i & Sb:2.843 &Sb:2a  &Ag@2a\\
\hline
\color{black}{ 635228} & \hyperref[subfig:635228]{Ga$_{2}$Ru} & 6 & 28 &  0.981 &  0.129 &  70 & 8b,16f & &&Ag@16d\&A@8b\\
 & & & & & & & & & &Ag@16d\&A@8a\\
\hline
\color{black}{ 196260} & \hyperref[subfig:196260]{ZrCu$_{4}$Ag} & 6 & 67 &  0.352 & -0.212 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
648286 & \hyperref[subfig:648286]{P$_{2}$W} & 6 & 32 &  0.071 & -0.663 &  12 & 4i &  P:2.193 & P:2a  &Ag@2c\&Ag@2a\\
\hline
\color{black}{ 238254} & \hyperref[subfig:238254]{Sb$_{2}$Os} & 6 & 36 &  1.023 &  0.346 &  58 & 4g,2a & Sb:2.857 &Sb:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
71998 & \hyperref[subfig:71998]{ScSiAu} & 6 & 36 &  0.336 & -0.530 & 187 & 1a,2h,1b,2i & Si:2.762 &Si:1d  &A1'@1e\&A1'@1d\\
 & & & & & & & & & &A1'@1e\&E''@1d\\
 & & & & & & & & & &E''@1e\&A1'@1d\\
 & & & & & & & & & &E''@1e\&E''@1d\\
\hline
\color{black}{ 609407} & \hyperref[subfig:609407]{SrAl$_{2}$} & 6 & 32 &  0.075 & -0.789 &  74 & 8h,4e & &&\\
\hline
\color{black}{ 419402} & \hyperref[subfig:419402]{RbSb$_{2}$} & 6 & 38 &  0.749 &  0.345 &  12 & 4i & Sb:2.818 &Sb:8j  &Ag@2a\\
\hline
647776 & \hyperref[subfig:647776]{Si$_{2}$Os} & 6 & 32 &  0.376 & -0.353 &  12 & 4i & Si:2.325 &Si:2c  &Ag@2c\&Ag@2a\\
\hline
\color{black}{ 612234} & \hyperref[subfig:612234]{YbNi$_{4}$Au} & 6 & 59 &  0.034 & -0.939 & 216 & 4c,16e,4a & &&A1@4d\&A1@4b\\
\hline
\color{black}{ 616209} & \hyperref[subfig:616209]{Be$_{5}$Co} & 6 & 19 &  0.629 & -0.059 & 216 & 4c,16e,4a & &&A1@4b\\
\hline
\color{black}{ 415196} & \hyperref[subfig:415196]{ErCdCu$_{4}$} & 6 & 65 &  0.378 & -0.689 & 216 & 16e,4d,4a & &&A1@4b\\
\hline
\color{black}{ 415195} & \hyperref[subfig:415195]{HoCdCu$_{4}$} & 6 & 65 &  0.408 & -0.637 & 216 & 16e,4d,4a & &&A1@4b\\
\hline
\color{black}{ 43652} & \hyperref[subfig:43652]{Sb$_{2}$Ru} & 6 & 36 &  0.641 & -0.000 &  58 & 4g,2a & Sb:2.830 &Sb:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
611576 & \hyperref[subfig:611576]{As$_{2}$W} & 6 & 32 &  0.037 & -0.731 &  12 & 4i & As:2.398 &As:2c  &Ag@2c\&Ag@2a\\
\hline
43898 & \hyperref[subfig:43898]{CrAs$_{2}$} & 6 & 32 &  0.031 & -0.626 &  12 & 4i & As:2.373 &As:2a  &Ag@2c\&Ag@2a\\
\hline
42578 & \hyperref[subfig:42578]{As$_{2}$Ru} & 6 & 36 &  0.985 &  0.230 &  58 & 4g,2a & As:2.360 &As:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
\color{black}{ 190546} & \hyperref[subfig:190546]{Na$_{2}$Cl} & 6 & 18 &  0.273 & -0.621 &  65 & 2d,4i,4j,2b & Cl:4.015 &Cl:4e  &Ag@2c\\
\hline
2526 & \hyperref[subfig:2526]{CrP$_{2}$} & 6 & 32 &  0.088 & -0.657 &  12 & 4i &  P:2.188 & P:2a  &Ag@2c\&Ag@2a\\
\hline
\color{black}{ 98666} & \hyperref[subfig:98666]{LiYGa$_{4}$} & 6 & 24 &  0.000 & -0.745 & 187 & 1a,2h,1b,2i & &&A1'@1e\&A1'@1d\\
 & & & & & & & & & &E''@1e\&A1'@1d\\
\hline
\color{black}{ 628018} & \hyperref[subfig:628018]{MgInCu$_{4}$} & 6 & 49 &  0.136 & -1.893 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
174577 & \hyperref[subfig:174577]{PbSe$_{2}$} & 6 & 32 &  0.153 & -0.355 & 140 & 8h,4a & Se:2.325 &Se:4d  &Ag@4d\\
 & & & & & & & & & &B1g@4d\\
\hline
\color{black}{ 191404} & \hyperref[subfig:191404]{ZrCu$_{5}$} & 6 & 67 &  0.352 & -0.337 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
187441 & \hyperref[subfig:187441]{ReN$_{2}$} & 6 & 34 &  0.343 & -0.327 &  12 & 4i &  N:1.405 & N:2c  &Ag@2c\\
\hline
75555 & \hyperref[subfig:75555]{BaTe$_{2}$} & 6 & 44 &  1.211 &  0.394 & 140 & 8h,4a & Te:2.772 &Te:4d  &Ag@4d\\
 & & & & & & & & & &B1g@4d\\
\hline
106001 & \hyperref[subfig:106001]{Te$_{2}$Ru} & 6 & 40 &  1.146 &  0.330 &  58 & 4g,2a & Te:2.864 &Te:2c  &Ag@2c\\
\hline
16820 & \hyperref[subfig:16820]{MoAs$_{2}$} & 6 & 32 &  0.058 & -0.715 &   5 & 4c & As:2.412 &As:2a  &A@2b\&A@2a\\
\hline
633072 & \hyperref[subfig:633072]{FeP$_{2}$} & 6 & 36 &  0.845 &  0.409 &  58 & 4g,2a &  P:2.167 & P:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
\color{black}{ 628189} & \hyperref[subfig:628189]{YbInCu$_{4}$} & 6 & 55 &  0.486 & -0.696 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
633866 & \hyperref[subfig:633866]{FeTe$_{2}$} & 6 & 40 &  0.542 &  0.011 &  58 & 4g,2a & Te:2.955 &Te:2c  &Ag@2c\\
\hline
\color{black}{ 417149} & \hyperref[subfig:417149]{YGaI} & 6 & 42 &  0.755 & -0.405 & 164 & 2d,2c &  I:4.178 & I:3f  &Ag@3e\\
\hline
65168 & \hyperref[subfig:65168]{FeAs$_{2}$} & 6 & 36 &  0.598 &  0.319 &  58 & 4g,2a & As:2.488 &As:2c  &Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
\color{black}{ 152560} & \hyperref[subfig:152560]{TbInCu$_{4}$} & 6 & 56 &  0.425 & -0.324 & 216 & 4c,16e,4a & &&A1@4d\\
\hline
201787 & \hyperref[subfig:201787]{V(MoS$_{2}$)$_{2}$} & 7 & 41 &  0.003 & -0.990 &  12 & 2a,4i &  S:3.026 & S:2c  &Ag@4f\&Au@2b\\
 & & & & & & & & & &Ag@4f\&Bu@2b\\
\hline
\color{black}{ 98990} & \hyperref[subfig:98990]{KB$_{6}$} & 7 & 27 &  0.782 &  0.782 & 221 & 1b,6e &  B:1.674 & B:3d  &\\
\hline
30734 & \hyperref[subfig:30734]{Rb$_{2}$Te$_{5}$} & 7 & 48 &  0.525 &  0.286 &  12 & 2a,4i,8j & Te:2.776 &Te:4h  &Ag@2d\&Au@2d\\
 & & & & & & & & & &Ag@2c\&Au@2c\\
\hline
\color{black}{ 20240} & \hyperref[subfig:20240]{SiB$_{6}$} & 7 & 22 &  1.424 &  0.440 & 221 & 1a,6f &  B:1.694 & B:12j &\\
\hline
190537 & \hyperref[subfig:190537]{NaCl$_{7}$} & 8 & 50 &  0.536 &  0.423 & 200 & 1a,6g,1b & Cl:2.053 &Cl:3d  &Ag@3d\\
\hline
79235 & \hyperref[subfig:79235]{SiRh} & 8 & 52 &  0.663 & -0.323 &  14 & 4e & Si:2.715 &Si:2c  &Ag@2a\\
\hline
\color{black}{ 245961} & \hyperref[subfig:245961]{Ge} & 8 & 32 &  0.000 & -0.720 & 148 & 6c,18f & &&Ag@9e\&A1g@3b\\
\hline
37073 & \hyperref[subfig:37073]{InP$_{3}$} & 8 & 36 &  0.000 & -0.900 & 166 & 6c,18h &  P:2.205 & P:18f &Ag@9e\&Au@9e\\
 & & & & & & & & & &A1g@3a\&A1u@3a\\
\hline
408030 & \hyperref[subfig:408030]{LaSi} & 8 & 60 &  0.007 & -0.835 &  63 & 8f,4c & Si:2.482 &Si:4c  &Ag@4a\\
\hline
640379 & \hyperref[subfig:640379]{TaInS$_{2}$} & 8 & 40 &  0.234 &  0.038 & 194 & 4f,2a,2b &  S:4.350 & S:2c  &A1'@2d\\
 & & & & & & & & & &E''@2d\\
\hline
16325 & \hyperref[subfig:16325]{Te$_{2}$AuI} & 8 & 60 &  0.050 & -0.458 &  51 & 2e,2c,4j & Te:2.778  I:6.660 &Te:2b   I:    &Ag@2b\\
\hline
26287 & \hyperref[subfig:26287]{NaNbSe$_{2}$} & 8 & 48 &  1.142 &  0.463 & 194 & 4f,2a,2b & Se:3.350 &Se:2c  &A1'@2d\\
 & & & & & & & & & &E''@2d\\
\hline
\color{black}{ 96089} & \hyperref[subfig:96089]{VAuS$_{2}$} & 8 & 56 &  0.488 & -0.035 & 194 & 2a,2c,4e &  S:2.861 & S:2b  &A1'@2d\\
\hline
\color{black}{ 413736} & \hyperref[subfig:413736]{LaGe} & 8 & 60 &  0.003 & -0.884 &  63 & 8f,4c & &&Ag@4b\\
\hline
613476 & \hyperref[subfig:613476]{CrB} & 8 & 36 &  0.001 & -1.388 & 141 & 8e &  B:1.638 & B:8d  &Ag@8c\&A2@4a\\
\hline
\color{black}{ 246170} & \hyperref[subfig:246170]{SiPt$_{3}$} & 8 & 68 &  0.003 & -0.468 &  12 & 4g,4h,4i & Si:3.413 &Si:2d  &Ag@4f\\
\hline
424240 & \hyperref[subfig:424240]{BW} & 8 & 36 &  0.021 & -3.354 & 141 & 8e &  B:1.883 & B:8d  &Ag@8c\&A2@4a\\
\hline
614793 & \hyperref[subfig:614793]{BMo} & 8 & 36 &  0.005 & -2.612 & 141 & 8e &  B:1.740 & B:8c  &Ag@8d\&A2@4b\\
\hline
185172 & \hyperref[subfig:185172]{InSe} & 8 & 36 &  0.495 &  0.495 & 194 & 4f & Se:3.784 &Se:6g  &A1'@2c\\
\hline
109036 & \hyperref[subfig:109036]{Si} & 8 & 32 &  0.554 & -0.512 & 148 & 6c,18f & Si:2.262 &Si:3b  &Ag@9e\&A1g@3b\\
\hline
240481 & \hyperref[subfig:240481]{Cs$_{2}$Pd(IBr$_{2}$)$_{2}$} & 9 & 70 &  0.598 &  0.136 & 139 & 4e,2a,8h,4d & Br:3.405  I:2.758 &Br:8i   I:2b  &B1@4d\&A1g@2b\\
\hline
\color{black}{ 181078} & \hyperref[subfig:181078]{Ca$_{6}$Ge$_{2}$O} & 9 & 74 &  0.331 &  0.287 & 225 & 24e,8c,4a & &&A1g@4b\\
\hline
81306 & \hyperref[subfig:81306]{Na(CuS)$_{4}$} & 9 & 69 &  0.264 &  0.264 & 164 & 2d,2c,1b &  S:2.084 & S:1a  &A1g@1a\\
\hline
\color{black}{ 626798} & \hyperref[subfig:626798]{CrSi$_{2}$} & 9 & 42 &  0.531 &  0.375 & 180 & 6j,3d & Si:2.476 &Si:6g  &A@3c\&B2@3c\\
 & & & & & & & & & &A@3a\&B2@3a\\
\hline
\color{black}{ 639879} & \hyperref[subfig:639879]{Li$_{5}$In$_{4}$} & 9 & 17 &  0.004 & -1.087 & 164 & 2d,2c,1b & &&A1g@1a\\
\hline
\color{black}{ 154596} & \hyperref[subfig:154596]{Nb$_{5}$Sb$_{4}$} & 9 & 75 &  0.000 & -0.756 &  87 & 2a,8h & Sb:3.577 &Sb:16i &Ag@2b\\
\hline
\color{black}{ 96026} & \hyperref[subfig:96026]{CrSi$_{2}$} & 9 & 42 &  0.532 &  0.373 & 181 & 3c,6i & Si:2.474 &Si:6h  &A@3d\&B2@3d\\
 & & & & & & & & & &A@3b\&B2@3b\\
\hline
\color{black}{ 652549} & \hyperref[subfig:652549]{Si$_{2}$W} & 9 & 42 &  0.515 & -0.015 & 180 & 6j,3d & Si:2.508 &Si:6g  &A@3c\&B2@3c\\
 & & & & & & & & & &A@3a\&B2@3a\\
\hline
248351 & \hyperref[subfig:248351]{Sr(RuO$_{3}$)$_{2}$} & 9 & 62 &  0.153 &  0.046 & 162 & 2d,1a,6k &  O:2.463 & O:3g  &A1u@1b\&Eg@1b\\
 & & & & & & & & & &A2u@1b\&Eg@1b\\
\hline
\color{black}{ 182116} & \hyperref[subfig:182116]{Si$_{2}$Mo} & 9 & 42 &  0.541 &  0.106 & 180 & 3c,6i & Si:2.558 &Si:6h  &A@3d\&B2@3d\\
 & & & & & & & & & &A@3b\&B2@3b\\
\hline
633091 & \hyperref[subfig:633091]{FePSe$_{3}$} & 10 & 62 &  0.354 &  0.340 & 148 & 6c,18f &  P:2.021 Se:3.519 & P:3b  Se:18f &A1g@3b\\
\hline
\color{black}{ 102868} & \hyperref[subfig:102868]{Cs$_{2}$In$_{3}$} & 10 & 54 &  0.172 & -0.005 & 119 & 8i,2d,2c,4e & &&B1@2d\&A2@2a\\
 & & & & & & & & & &B1@2c\&A2@2a\\
\hline
260563 & \hyperref[subfig:260563]{Sr(InP)$_{2}$} & 10 & 52 &  0.399 &  0.399 & 194 & 4f,2a &  P:4.541 & P:6g  &A1'@2d\\
\hline
409381 & \hyperref[subfig:409381]{Rb$_{2}$As$_{3}$} & 10 & 66 &  0.400 &  0.393 &  69 & 8f,8h,8i,16n & As:2.375 &As:8g  &B3u@4a\\
\hline
602341 & \hyperref[subfig:602341]{NiPS$_{3}$} & 10 & 66 &  0.001 & -0.134 &  12 & 4g,4i,8j &  P:2.154  S:3.347 & P:2a   S:8j  &Au@2a\\
 & & & & & & & & & &Bu@2a\\
\hline
\color{black}{ 160496} & \hyperref[subfig:160496]{K$_{2}$Ga$_{3}$} & 10 & 54 &  0.386 &  0.115 & 139 & 8i,4e,4d & &&Ag@4c\&B2g@2a\\
\hline
422525 & \hyperref[subfig:422525]{Ca(GaP)$_{2}$} & 10 & 52 &  0.900 &  0.220 & 194 & 4f,2a &  P:4.370 & P:6g  &A1'@2c\\
\hline
61392 & \hyperref[subfig:61392]{FePS$_{3}$} & 10 & 62 &  0.339 &  0.293 &  12 & 4g,4i,8j &  P:2.174  S:3.409 & P:2a   S:4i  &Ag@2a\\
 & & & & & & & & & &Bg@2a\\
\hline
\color{black}{ 639449} & \hyperref[subfig:639449]{Ho$_{3}$Ni$_{2}$} & 10 & 94 &  0.000 & -0.789 &  12 & 4i & &&Ag@2c\\
\hline
\color{black}{ 646858} & \hyperref[subfig:646858]{Tb$_{3}$Ni$_{2}$} & 10 & 94 &  0.009 & -0.755 &  12 & 4i & &&Ag@2c\\
\hline
\color{black}{ 2334} & \hyperref[subfig:2334]{Dy$_{3}$Ni$_{2}$} & 10 & 94 &  0.000 & -0.794 &  12 & 4i & &&Ag@2c\\
\hline
\color{black}{ 190543} & \hyperref[subfig:190543]{Na$_{3}$Cl$_{2}$} & 10 & 34 &  0.752 & -0.318 &  83 & 4k,1a,1d,4j & Cl:3.575 &Cl:4j  &Ag@1b\\
\hline
409382 & \hyperref[subfig:409382]{Cs$_{2}$As$_{3}$} & 10 & 66 &  0.426 &  0.426 &  69 & 8f,8h,8i,16n & As:2.369 &As:8g  &B3u@4a\\
\hline
646145 & \hyperref[subfig:646145]{NiPSe$_{3}$} & 10 & 66 &  0.001 & -0.215 &  12 & 4g,4i,8j &  P:2.241 Se:3.520 & P:2a  Se:8j  &Au@2a\\
 & & & & & & & & & &Bu@2a\\
\hline
68014 & \hyperref[subfig:68014]{Y$_{4}$CI$_{5}$} & 10 & 83 &  0.044 & -0.087 &  12 & 2d,4i,2b &  I:3.984 & I:4i  &Au@2a\\
 & & & & & & & & & &Bu@2a\\
\hline
280027 & \hyperref[subfig:280027]{Ba$_{3}$(LiAs)$_{4}$} & 11 & 54 &  0.005 & -0.009 &  71 & 2a,4j,8l,4h,4i & As:2.487 &As:2c  &Ag@2c\\
 & & & & & & & & & &B3g@2c\\
\hline
\color{black}{ 58001} & \hyperref[subfig:58001]{Al$_{8}$Mo$_{3}$} & 11 & 42 &  0.054 & -0.095 &  12 & 2a,4i & &&Ag@2c\&Ag@2b\\
 & & & & & & & & & &Ag@2c\&Bg@2b\\
\hline
162061 & \hyperref[subfig:162061]{Cu$_{2}$As$_{2}$O$_{7}$} & 11 & 74 &  0.020 & -0.184 &  12 & 2a,4h,4i,8j & As:3.331  O:2.463 &As:     O:2d  &Au@2d\\
 & & & & & & & & & &Bu@2d\\
\hline
27436 & \hyperref[subfig:27436]{Cu$_{2}$P$_{2}$O$_{7}$} & 11 & 74 &  0.001 & -0.261 &  12 & 2a,4h,4i,8j &  P:3.085  O:2.434 & P:     O:4i  &Au@2d\\
 & & & & & & & & & &Bu@2d\\
\hline
40823 & \hyperref[subfig:40823]{Ir$_{3}$Se$_{8}$} & 11 & 75 &  0.049 & -0.466 & 148 & 6c,9e,18f & Se:2.232 &Se:9d  &Ag@9d\\
\hline
\color{black}{ 66002} & \hyperref[subfig:66002]{CaGaGe} & 12 & 68 &  0.070 & -1.108 & 194 & 4f,2a,2b & &&A1'@2c\\
\hline
42569 & \hyperref[subfig:42569]{NiAs$_{2}$} & 12 & 80 &  0.001 & -0.466 & 205 & 8c,4a & As:2.399 &As:4b  &A1g@4b\\
\hline
\color{black}{ 624977} & \hyperref[subfig:624977]{ScCoSn} & 12 & 64 &  0.032 & -0.184 &  62 & 4c & &&Ag@4b\\
\hline
\color{black}{ 636739} & \hyperref[subfig:636739]{TbGeIr} & 12 & 88 &  0.232 & -0.573 &  62 & 4c & &&Ag@4b\\
\hline
\color{black}{ 54415} & \hyperref[subfig:54415]{DyCoSn} & 12 & 88 &  0.004 & -0.321 &  62 & 4c & &&Ag@4b\\
\hline
24801 & \hyperref[subfig:24801]{SiAs$_{2}$} & 12 & 56 &  0.356 & -0.971 & 205 & 8c,4a & Si:4.259 As:2.416 &Si:24d As:4b  &A1g@4b\\
\hline
610769 & \hyperref[subfig:610769]{LaAs$_{2}$} & 12 & 84 &  0.742 &  0.183 &  14 & 4e & As:2.525 &As:4e  &Ag@2b\\
\hline
412793 & \hyperref[subfig:412793]{RbNdTe$_{4}$} & 12 & 88 &  0.948 &  0.203 & 125 & 2a,8m,2b & Te:2.777 &Te:4h  &A1@2d\&B2@2d\\
 & & & & & & & & & &B1@2d\&A2@2d\\
 & & & & & & & & & &B2@2d\&A2@2d\\
 & & & & & & & & & &A1@2c\&B2@2c\\
 & & & & & & & & & &B1@2c\&A2@2c\\
\hline
611219 & \hyperref[subfig:611219]{PrAs$_{2}$} & 12 & 84 &  0.677 & -0.067 &  14 & 4e & As:2.490 &As:4e  &Ag@2b\\
\hline
43101 & \hyperref[subfig:43101]{As$_{2}$Pd} & 12 & 80 &  0.235 & -0.493 & 205 & 8c,4a & As:2.426 &As:4b  &A1g@4b\\
\hline
24202 & \hyperref[subfig:24202]{OsSe$_{2}$} & 12 & 80 &  0.573 &  0.205 & 205 & 8c,4a & Se:2.431 &Se:4b  &A1g@4b\\
\hline
300225 & \hyperref[subfig:300225]{Te$_{2}$Os} & 12 & 80 &  0.090 & -0.105 & 205 & 8c,4a & Te:2.817 &Te:4b  &A1g@4b\\
\hline
650607 & \hyperref[subfig:650607]{RuSe$_{2}$} & 12 & 80 &  0.797 &  0.439 & 205 & 8c,4a & Se:2.445 &Se:4b  &A1g@4b\\
\hline
24187 & \hyperref[subfig:24187]{OsS$_{2}$} & 12 & 80 &  0.406 &  0.174 & 205 & 8c,4a &  S:2.209 & S:4b  &A1g@4b\\
\hline
419345 & \hyperref[subfig:419345]{NdS$_{2}$} & 12 & 92 &  0.815 &  0.290 &  14 & 4e &  S:2.134 & S:2c  &Ag@2c\\
\hline
412792 & \hyperref[subfig:412792]{KNdTe$_{4}$} & 12 & 88 &  0.978 &  0.190 & 125 & 2a,8m,2b & Te:2.780 &Te:4h  &A1@2d\&B2@2d\\
 & & & & & & & & & &B1@2d\&A2@2d\\
 & & & & & & & & & &B2@2d\&A2@2d\\
 & & & & & & & & & &A1@2c\&B2@2c\\
 & & & & & & & & & &B1@2c\&A2@2c\\
\hline
75029 & \hyperref[subfig:75029]{CuBIr} & 12 & 92 &  0.009 & -0.701 &  43 & 16b &  B:3.200 & B:16b &A@8a\\
\hline
\color{black}{ 420415} & \hyperref[subfig:420415]{ScCoSi} & 12 & 64 &  0.055 & -0.369 &  62 & 4c & Si:3.672 &Si:4a  &Ag@4a\\
\hline
65169 & \hyperref[subfig:65169]{Te$_{2}$Ru} & 12 & 80 &  0.376 &  0.096 & 205 & 8c,4a & Te:2.810 &Te:4b  &A1g@4b\\
\hline
\color{black}{ 88166} & \hyperref[subfig:88166]{HoGeIr} & 12 & 88 &  0.070 & -0.676 &  62 & 4c & &&Ag@4a\\
\hline
\color{black}{ 280231} & \hyperref[subfig:280231]{LaTeAs} & 12 & 88 &  0.139 &  0.077 &  62 & 4c & As:2.635 Te:4.008 &As:4a  Te:4b  &Ag@4a\\
\hline
610026 & \hyperref[subfig:610026]{CoAs$_{2}$} & 12 & 76 &  0.203 &  0.142 &  14 & 4e & As:2.518 &As:4e  &Ag@2d\\
\hline
\color{black}{ 82549} & \hyperref[subfig:82549]{NdGeRh} & 12 & 96 &  0.121 & -0.587 &  62 & 4c & &&Ag@4b\\
\hline
24203 & \hyperref[subfig:24203]{As$_{2}$Pt} & 12 & 80 &  1.048 &  0.263 & 205 & 8c,4a & As:2.377 &As:4b  &A1g@4b\\
\hline
\color{black}{ 107587} & \hyperref[subfig:107587]{Bi$_{3}$Te$_{2}$S} & 12 & 66 &  0.042 & -0.029 & 164 & 2d,2c &  S:3.585 Te:4.385 & S:3e  Te:6i  &Ag@3f\\
\hline
\color{black}{ 633674} & \hyperref[subfig:633674]{ZrFeSi} & 12 & 96 &  0.097 & -0.313 &  62 & 4c & Si:3.721 &Si:4a  &Ag@4a\\
\hline
\color{black}{ 88167} & \hyperref[subfig:88167]{ErGeIr} & 12 & 88 &  0.183 & -0.279 &  62 & 4c & &&Ag@4a\\
\hline
633405 & \hyperref[subfig:633405]{FeSbTe} & 12 & 76 &  0.338 &  0.201 &  14 & 4e & Te:3.631 Sb:3.557 &Te:4e  Sb:2a  &Ag@2d\\
\hline
\color{black}{ 88213} & \hyperref[subfig:88213]{TbCoSi} & 12 & 88 &  0.015 & -0.419 &  62 & 4c & Si:3.730 &Si:4b  &Ag@4b\\
\hline
\color{black}{ 636724} & \hyperref[subfig:636724]{PrGeIr} & 12 & 96 &  0.028 & -0.391 &  62 & 4c & &&Ag@4a\\
\hline
\color{black}{ 93221} & \hyperref[subfig:93221]{TbSiIr} & 12 & 88 &  0.032 & -0.744 &  62 & 4c & Si:3.851 &Si:4a  &Ag@4a\\
\hline
\color{black}{ 428472} & \hyperref[subfig:428472]{ScCoGe} & 12 & 64 &  0.070 & -0.493 &  62 & 4c & &&Ag@4a\\
\hline
\color{black}{ 424397} & \hyperref[subfig:424397]{Bi$_{2}$Ir} & 12 & 76 &  0.299 & -0.217 &  14 & 4e & &&Ag@2d\\
\hline
391204 & \hyperref[subfig:391204]{KPrTe$_{4}$} & 12 & 88 &  0.971 &  0.206 & 125 & 2a,8m,2b & Te:2.776 &Te:4h  &A1@2d\&B2@2d\\
 & & & & & & & & & &B1@2d\&A2@2d\\
 & & & & & & & & & &B2@2d\&A2@2d\\
 & & & & & & & & & &A1@2c\&B2@2c\\
 & & & & & & & & & &B1@2c\&A2@2c\\
\hline
\color{black}{ 152569} & \hyperref[subfig:152569]{YbGaGe} & 12 & 60 &  0.060 & -1.070 & 194 & 4f,2a,2b & &&A1'@2c\\
\hline
30692 & \hyperref[subfig:30692]{SiP$_{2}$} & 12 & 56 &  0.919 & -0.832 & 205 & 8c,4a & Si:4.017  P:2.156 &Si:24d  P:4b  &A1g@4b\\
\hline
\color{black}{ 428475} & \hyperref[subfig:428475]{ScGeRh} & 12 & 64 &  0.026 & -0.792 &  62 & 4c & &&Ag@4a\\
\hline
\color{black}{ 43105} & \hyperref[subfig:43105]{Sb$_{2}$Pt} & 12 & 80 &  0.084 & -0.089 & 205 & 8c,4a & Sb:2.789 &Sb:4b  &A1g@4b\\
\hline
\color{black}{ 636748} & \hyperref[subfig:636748]{TmGeIr} & 12 & 88 &  0.103 & -0.811 &  62 & 4c & &&Ag@4b\\
\hline
\color{black}{ 79596} & \hyperref[subfig:79596]{ScSiRh} & 12 & 64 &  0.040 & -0.738 &  62 & 4c & Si:3.783 &Si:4c  &Ag@4a\\
\hline
\color{black}{ 43501} & \hyperref[subfig:43501]{Sb$_{2}$Rh} & 12 & 76 &  0.124 &  0.031 &  14 & 4e & Sb:2.829 &Sb:4e  &Ag@2d\\
\hline
\color{black}{ 88272} & \hyperref[subfig:88272]{DyCoSi} & 12 & 88 &  0.002 & -0.434 &  62 & 4c & Si:3.731 &Si:4a  &Ag@4a\\
\hline
412794 & \hyperref[subfig:412794]{RbPrTe$_{4}$} & 12 & 88 &  0.959 &  0.221 & 125 & 2a,8m,2b & Te:2.778 &Te:4h  &A1@2d\&B2@2d\\
 & & & & & & & & & &B1@2d\&A2@2d\\
 & & & & & & & & & &B2@2d\&A2@2d\\
 & & & & & & & & & &A1@2c\&B2@2c\\
 & & & & & & & & & &B1@2c\&A2@2c\\
\hline
\color{black}{ 412708} & \hyperref[subfig:412708]{LuGeIr} & 12 & 88 &  0.033 & -0.783 &  62 & 4c & &&Ag@4a\\
\hline
611271 & \hyperref[subfig:611271]{As$_{2}$Rh} & 12 & 76 &  0.503 &  0.479 &  14 & 4e & As:2.489 &As:4e  &Ag@2d\\
\hline
\color{black}{ 291479} & \hyperref[subfig:291479]{Si} & 12 & 48 &  0.546 &  0.468 &  63 & 8f & Si:2.303 &Si:4c  &\\
\hline
\color{black}{ 163343} & \hyperref[subfig:163343]{CeZnGe} & 12 & 108 &  0.070 & -1.247 & 194 & 4f,2a,2b & &&A1'@2c\\
 & & & & & & & & & &E''@2c\\
\hline
\color{black}{ 237303} & \hyperref[subfig:237303]{SrNiGe} & 12 & 96 &  0.140 & -0.384 &  62 & 4c & &&Ag@4a\\
\hline
610996 & \hyperref[subfig:610996]{NdAs$_{2}$} & 12 & 84 &  0.669 & -0.083 &  14 & 4e & As:2.476 &As:4e  &Ag@2b\\
\hline
\color{black}{ 102867} & \hyperref[subfig:102867]{CsIn$_{3}$} & 12 & 54 &  0.261 &  0.060 & 119 & 4f,2a,8i,2b & &&A2@2c\&B1@2b\\
 & & & & & & & & & &A2@2c\&B1@2a\\
\hline
633475 & \hyperref[subfig:633475]{FeSe$_{2}$} & 12 & 80 &  0.587 &  0.486 & 205 & 8c,4a & Se:2.405 &Se:4b  &A1g@4b\\
\hline
633399 & \hyperref[subfig:633399]{FeSbSe} & 12 & 76 &  0.343 &  0.178 &  14 & 4e & Se:3.463 Sb:3.374 &Se:4e  Sb:2a  &Ag@2d\\
\hline
610526 & \hyperref[subfig:610526]{FeAsSe} & 12 & 76 &  0.463 &  0.260 &  14 & 4e & Se:3.289 As:3.207 &Se:4e  As:2a  &Ag@2d\\
\hline
647944 & \hyperref[subfig:647944]{PrP$_{2}$} & 12 & 84 &  0.648 & -0.129 &  14 & 4e &  P:2.389 & P:4e  &Ag@2b\\
\hline
409185 & \hyperref[subfig:409185]{HoP$_{5}$} & 12 & 68 &  0.727 &  0.078 &  11 & 4f,2e &  P:2.168 & P:4f  &Ag@2d\&Ag@2b\\
\hline
421335 & \hyperref[subfig:421335]{GdS$_{2}$} & 12 & 84 &  0.953 &  0.293 &  14 & 4e &  S:2.140 & S:2c  &Ag@2c\\
\hline
38316 & \hyperref[subfig:38316]{CoP$_{2}$} & 12 & 76 &  0.352 &  0.346 &  14 & 4e &  P:2.212 & P:4e  &Ag@2d\\
\hline
620416 & \hyperref[subfig:620416]{CdSe$_{2}$} & 12 & 96 &  0.654 &  0.499 & 205 & 8c,4a & Se:2.521 &Se:4b  &A1g@4b\\
\hline
358 & \hyperref[subfig:358]{NdP$_{5}$} & 12 & 72 &  0.733 & -0.127 &  11 & 4f,2e &  P:2.162 & P:4f  &Ag@2d\&Ag@2b\\
\hline
\color{black}{ 34450} & \hyperref[subfig:34450]{CuAsS} & 12 & 88 &  0.108 & -0.171 &  62 & 4c & As:2.498  S:3.831 &As:4b   S:8d  &Ag@4b\\
\hline
633093 & \hyperref[subfig:633093]{FePSe} & 12 & 76 &  0.565 &  0.338 &  14 & 4e & Se:3.210  P:3.114 &Se:4e   P:2a  &Ag@2d\\
\hline
160624 & \hyperref[subfig:160624]{RhN$_{2}$} & 12 & 76 &  0.067 & -0.746 &  14 & 4e &  N:1.307 & N:4e  &Ag@2a\\
\hline
\color{black}{ 191245} & \hyperref[subfig:191245]{PdN$_{2}$} & 12 & 80 &  0.170 &  0.160 & 205 & 8c,4a &  N:1.213 & N:4b  &\\
\hline
\color{black}{ 102863} & \hyperref[subfig:102863]{CsGa$_{3}$} & 12 & 54 &  0.153 & -0.135 & 119 & 4f,2a,8i,2b & &&A2@2c\&B1@2b\\
 & & & & & & & & & &A2@2c\&B1@2a\\
\hline
82721 & \hyperref[subfig:82721]{ReTeS} & 12 & 76 &  0.670 &  0.147 & 216 & 16e & Te:3.486  S:3.403 &Te:24g  S:24g &E@4b\\
 & & & & & & & & & &E@4a\\
\hline
24774 & \hyperref[subfig:24774]{HgO$_{2}$} & 12 & 96 &  0.834 &  0.365 &  61 & 8c,4a &  O:1.490 & O:4b  &Ag@4b\\
\hline
22221 & \hyperref[subfig:22221]{NiP$_{2}$} & 12 & 80 &  0.402 & -0.204 & 205 & 8c,4a &  P:2.121 & P:4b  &A1g@4b\\
\hline
648826 & \hyperref[subfig:648826]{PdSe$_{2}$} & 12 & 88 &  0.560 & -0.080 &  61 & 8c,4a & Se:2.363 &Se:4b  &Ag@4b\\
\hline
\color{black}{ 152623} & \hyperref[subfig:152623]{LaZnSn} & 12 & 108 &  0.028 & -0.693 & 194 & 4f,2a,2b & &&A1'@2c\\
 & & & & & & & & & &E''@2c\\
\hline
409183 & \hyperref[subfig:409183]{SmP$_{5}$} & 12 & 72 &  0.761 & -0.033 &  11 & 4f,2e &  P:2.161 & P:4f  &Ag@2d\&Ag@2b\\
\hline
\color{black}{ 166387} & \hyperref[subfig:166387]{SrGaSn} & 12 & 68 &  0.021 & -0.974 & 194 & 4f,2a,2b & &&A1'@2c\\
\hline
633086 & \hyperref[subfig:633086]{FePS} & 12 & 76 &  0.530 &  0.325 &  14 & 4e &  S:3.122  P:3.034 & S:4e   P:2a  &Ag@2d\\
\hline
32530 & \hyperref[subfig:32530]{LaSe$_{2}$} & 12 & 92 &  0.603 &  0.218 &  14 & 4e & Se:2.462 &Se:2c  &Ag@2c\\
\hline
409186 & \hyperref[subfig:409186]{TmP$_{5}$} & 12 & 68 &  0.670 & -0.287 &  11 & 4f,2e &  P:2.158 & P:4f  &Ag@2d\&Ag@2b\\
\hline
616892 & \hyperref[subfig:616892]{BiOsSe} & 12 & 76 &  0.598 &  0.376 &  14 & 4e & Se:3.627 &Se:4e  &Ag@2d\\
\hline
409188 & \hyperref[subfig:409188]{YP$_{5}$} & 12 & 72 &  0.736 &  0.106 &  11 & 4f,2e &  P:2.165 & P:4f  &Ag@2d\&Ag@2b\\
\hline
422672 & \hyperref[subfig:422672]{TbS$_{2}$} & 12 & 84 &  0.989 &  0.286 &  14 & 4e &  S:2.141 & S:2c  &Ag@2c\\
\hline
41858 & \hyperref[subfig:41858]{CoAsS} & 12 & 80 &  0.046 & -0.404 &  14 & 2d,2a,4e & As:2.204  S:2.204 &As:2b   S:2c  &Ag@2c\&Ag@2b\\
\hline
409184 & \hyperref[subfig:409184]{DyP$_{5}$} & 12 & 68 &  0.745 &  0.072 &  11 & 4f,2e &  P:2.160 & P:4f  &Ag@2d\&Ag@2b\\
\hline
409182 & \hyperref[subfig:409182]{PrP$_{5}$} & 12 & 72 &  0.708 & -0.175 &  11 & 4f,2e &  P:2.166 & P:4f  &Ag@2d\&Ag@2b\\
\hline
422673 & \hyperref[subfig:422673]{ErS$_{2}$} & 12 & 84 &  1.135 &  0.337 &  14 & 4e &  S:2.146 & S:2c  &Ag@2c\\
\hline
\color{black}{ 20664} & \hyperref[subfig:20664]{KGa$_{3}$} & 12 & 54 &  0.391 &  0.226 & 119 & 8i,2d,2c,4e & &&B1@2d\&A2@2a\\
 & & & & & & & & & &B1@2c\&A2@2a\\
\hline
409187 & \hyperref[subfig:409187]{LuP$_{5}$} & 12 & 68 &  0.693 &  0.135 &  11 & 4f,2e &  P:2.162 & P:4f  &Ag@2d\&Ag@2b\\
\hline
240755 & \hyperref[subfig:240755]{IrN$_{2}$} & 12 & 76 &  0.929 &  0.325 &  14 & 4e &  N:1.430 & N:4e  &Ag@2a\\
\hline
92525 & \hyperref[subfig:92525]{PrS$_{2}$} & 12 & 92 &  0.809 &  0.297 &  14 & 4e &  S:2.135 & S:2c  &Ag@2c\\
\hline
414619 & \hyperref[subfig:414619]{NdSe$_{2}$} & 12 & 92 &  0.408 & -0.172 &  14 & 4e & Se:2.476 &Se:2c  &Ag@2c\\
\hline
413527 & \hyperref[subfig:413527]{PrSe$_{2}$} & 12 & 92 &  0.368 & -0.172 &  14 & 4e & Se:2.462 &Se:2c  &Ag@2c\\
\hline
\color{black}{ 103943} & \hyperref[subfig:103943]{RbGa$_{3}$} & 12 & 54 &  0.424 &  0.252 & 119 & 4f,2a,8i,2b & &&A2@2d\&B1@2b\\
 & & & & & & & & & &A2@2d\&B1@2a\\
\hline
\color{black}{ 615734} & \hyperref[subfig:615734]{YbB$_{12}$} & 13 & 44 &  0.053 & -0.373 & 225 & 48i,4a &  B:1.669 & B:24d &\\
\hline
\color{black}{ 624284} & \hyperref[subfig:624284]{Nb$_{7}$Co$_{6}$} & 13 & 131 &  0.002 & -0.529 & 166 & 6c,3a,18h & &&A1g@3b\&Eu@3b\\
\hline
425778 & \hyperref[subfig:425778]{Ba(P$_{2}$Au)$_{2}$} & 14 & 104 &  0.635 &  0.247 &  70 & 32h,8b,16g &  P:2.208 & P:16g &Ag@16c\\
\hline
247425 & \hyperref[subfig:247425]{Sc$_{2}$Si$_{2}$Pt$_{3}$} & 14 & 88 &  0.113 & -0.757 &  55 & 2a,4g,4h & Si:2.776 &Si:2b  &Ag@2d\\
\hline
426082 & \hyperref[subfig:426082]{Eu$_{2}$Zn$_{2}$P$_{3}$} & 14 & 114 &  0.041 & -0.703 &  12 & 4i &  P:2.255 & P:2a  &Ag@2a\\
\hline
406949 & \hyperref[subfig:406949]{Bi$_{4}$RuI$_{2}$} & 14 & 84 &  0.222 &  0.201 &  87 & 8h,4e &  I:4.252 & I:4c  &Ag@2b\&Bg@2a\\
\hline
\color{black}{ 82533} & \hyperref[subfig:82533]{Sr$_{3}$(GeN)$_{2}$} & 14 & 96 &  0.026 & -1.477 &  11 & 2e &  N:2.976 & N:2e  &Ag@2a\\
\hline
262413 & \hyperref[subfig:262413]{Sr$_{2}$Zn$_{2}$As$_{3}$} & 14 & 118 &  0.132 &  0.128 &  12 & 4i & As:2.496 &As:2a  &Ag@2a\\
\hline
\color{black}{ 2150} & \hyperref[subfig:2150]{Er$_{3}$Ni$_{2}$} & 15 & 141 &  0.010 & -0.281 & 148 & 6c,3b,18f & &&A1g@3a\\
\hline
6031 & \hyperref[subfig:6031]{Sb$_{2}$I$_{2}$F$_{11}$} & 15 & 101 &  2.361 &  2.283 &   5 & 4c,2b &  I:2.557 Sb:3.975  F:2.535 & I:2a  Sb:2b   F:4c  &A@2a\\
\hline
\color{black}{ 639447} & \hyperref[subfig:639447]{Ho$_{3}$Ni$_{2}$} & 15 & 141 &  0.023 & -0.290 & 148 & 6c,18f,3a & &&A1g@3b\\
\hline
\color{black}{ 281462} & \hyperref[subfig:281462]{Ca$_{6}$Cr$_{2}$HN$_{6}$} & 15 & 103 &  0.505 &  0.478 & 148 & 6c,18f,3a &  N:3.023 & N:18f &\\
\hline
\color{black}{ 10509} & \hyperref[subfig:10509]{Mn$_{4}$Al$_{11}$} & 15 & 61 &  0.232 &  0.095 &   2 & 1a,2i & &&\\
\hline
173357 & \hyperref[subfig:173357]{Ba$_{4}$Fe$_{2}$S$_{4}$I$_{5}$} & 15 & 115 &  0.099 & -0.008 &  87 & 2a,8h,4d &  I:4.195  S:3.683 & I:16i  S:16i &Ag@4c\&Ag@4c\\
 & & & & & & & & & &Ag@4c\&Bg@4c\\
 & & & & & & & & & &Bg@4c\&Bg@4c\\
\hline
\color{black}{ 35200} & \hyperref[subfig:35200]{TcP$_{3}$} & 16 & 88 &  0.503 &  0.436 &  62 & 4c &  P:2.197 & P:4b  &Ag@4b\\
\hline
\color{black}{ 34048} & \hyperref[subfig:34048]{CoSb$_{3}$} & 16 & 96 &  0.135 &  0.135 & 204 & 24g,8c & Sb:2.895 &Sb:12d &\\
\hline
\color{black}{ 34050} & \hyperref[subfig:34050]{Sb$_{3}$Ir} & 16 & 96 &  0.196 &  0.196 & 204 & 24g,8c & Sb:2.846 &Sb:12d &\\
\hline
\color{black}{ 76500} & \hyperref[subfig:76500]{Tl$_{2}$(CdSb)$_{3}$} & 16 & 114 &  0.346 &  0.026 &  12 & 4i & Sb:2.826 &Sb:2c  &Ag@2c\\
\hline
78364 & \hyperref[subfig:78364]{LiSi} & 16 & 40 &  0.667 & -0.018 &  88 & 16f & Si:2.417 &Si:16f &Ag@8c\\
\hline
\color{black}{ 647985} & \hyperref[subfig:647985]{ReP$_{3}$} & 16 & 88 &  0.236 &  0.220 &  62 & 4c &  P:2.198 & P:4c  &Ag@4b\\
\hline
\color{black}{ 52831} & \hyperref[subfig:52831]{CdSb} & 16 & 136 &  0.330 &  0.068 &  61 & 8c & Sb:2.811 &Sb:4a  &Ag@4a\\
\hline
\color{black}{ 162107} & \hyperref[subfig:162107]{RhN$_{3}$} & 16 & 96 &  0.228 & -0.057 & 204 & 24g,8c &  N:1.465 & N:12d &\\
\hline
427612 & \hyperref[subfig:427612]{ZnAs} & 16 & 136 &  0.643 &  0.347 &  61 & 8c & As:2.429 &As:4a  &Ag@4a\\
\hline
\color{black}{ 23628} & \hyperref[subfig:23628]{SrP$_{3}$} & 16 & 100 &  0.359 &  0.359 &  12 & 8j,4i &  P:2.188 & P:8j  &\\
\hline
\color{black}{ 55514} & \hyperref[subfig:55514]{In$_{3}$Ru} & 16 & 68 &  0.604 &  0.191 & 136 & 4f,4c,8j & &&Ag@2b\\
\hline
27159 & \hyperref[subfig:27159]{NiP} & 16 & 120 &  0.046 & -0.461 &  61 & 8c &  P:2.429 & P:4a  &Ag@4b\\
\hline
\color{black}{ 601137} & \hyperref[subfig:601137]{ZnSb} & 16 & 136 &  0.435 &  0.054 &  61 & 8c & Sb:2.811 &Sb:4a  &Ag@4a\\
\hline
\color{black}{ 635229} & \hyperref[subfig:635229]{Ga$_{3}$Ru} & 16 & 68 &  0.742 &  0.364 & 136 & 4f,4c,8j & &&Ag@2b\\
\hline
66024 & \hyperref[subfig:66024]{K$_{5}$Te$_{3}$} & 16 & 126 &  0.198 &  0.106 &  87 & 8h,4e,4d & Te:2.840 &Te:2a  &Ag@2a\\
\hline
\color{black}{ 634441} & \hyperref[subfig:634441]{Ga$_{3}$Ir} & 16 & 72 &  0.119 & -0.034 & 136 & 4f,4c,8j & &&Ag@2b\&Ag@2a\\
\hline
\color{black}{ 103448} & \hyperref[subfig:103448]{Ga$_{3}$Fe} & 16 & 68 &  0.719 &  0.458 & 136 & 4f,4c,8j & &&Ag@2b\\
\hline
\color{black}{ 51976} & \hyperref[subfig:51976]{Mg$_{3}$In} & 16 & 36 &  0.005 & -1.580 & 166 & 6c,18h & &&A1g@3b\&A1g@3a\\
\hline
\color{black}{ 635023} & \hyperref[subfig:635023]{Ga$_{3}$Os} & 16 & 68 &  0.417 & -0.056 & 136 & 4c,8j,8i & &&Ag@2a\\
\hline
\color{black}{ 648855} & \hyperref[subfig:648855]{SiPd$_{3}$} & 16 & 136 &  0.002 & -0.652 &  62 & 8d,4c & Si:3.685 &Si:4c  &Ag@4b\\
\hline
\color{black}{ 638878} & \hyperref[subfig:638878]{Hf$_{3}$Sb} & 16 & 68 &  0.005 & -0.221 &  82 & 8g & Sb:4.267 &Sb:8g  &A@2c\&A@2b\\
\hline
\color{black}{ 640899} & \hyperref[subfig:640899]{P$_{3}$Ir} & 16 & 96 &  0.426 &  0.123 & 204 & 24g,8c &  P:2.228 & P:12d &\\
\hline
\color{black}{ 408324} & \hyperref[subfig:408324]{Li$_{3}$CaMnN$_{3}$} & 16 & 70 &  0.123 &  0.123 & 148 & 6c,18f &  N:2.990 & N:18f &\\
\hline
96509 & \hyperref[subfig:96509]{LiSi} & 16 & 40 &  0.657 & -0.038 &  88 & 16f & Si:2.419 &Si:16f &Ag@8c\\
\hline
\color{black}{ 103448} & \hyperref[subfig:103448]{Ga$_{3}$Fe} & 16 & 68 &  0.719 &  0.458 & 136 & 4f,4c,8j & &&Ag@2b\\
\hline
83664 & \hyperref[subfig:83664]{Al$_{2}$(FeSi)$_{3}$} & 16 & 84 &  0.104 &  0.016 &   2 & 2i & Si:2.424 &Si:1f  &Ag@1g\&Ag@1c\\
\hline
\color{black}{ 23080} & \hyperref[subfig:23080]{La(FeAs$_{3}$)$_{4}$} & 17 & 103 &  0.613 &  0.545 & 204 & 24g,2a,8c & As:2.571 &As:12e &\\
\hline
\color{black}{ 610010} & \hyperref[subfig:610010]{Ce(As$_{3}$Os)$_{4}$} & 17 & 103 &  0.776 &  0.257 & 204 & 24g,2a,8c & As:2.626 &As:12e &\\
\hline
\color{black}{ 610521} & \hyperref[subfig:610521]{Pr(FeAs$_{3}$)$_{4}$} & 17 & 103 &  0.350 &  0.228 & 204 & 24g,2a,8c & As:2.560 &As:12e &\\
\hline
\color{black}{ 610013} & \hyperref[subfig:610013]{Ce(As$_{3}$Ru)$_{4}$} & 17 & 103 &  0.496 & -0.006 & 204 & 24g,2a,8c & As:2.615 &As:12e &\\
\hline
\color{black}{ 183088} & \hyperref[subfig:183088]{Nd(Sb$_{3}$Os)$_{4}$} & 17 & 103 &  0.829 &  0.254 & 204 & 24g,2a,8c & Sb:2.901 &Sb:12d &\\
\hline
\color{black}{ 79927} & \hyperref[subfig:79927]{Nd(FeSb$_{3}$)$_{4}$} & 17 & 103 &  0.708 &  0.383 & 204 & 24g,2a,8c & Sb:2.921 &Sb:12d &\\
\hline
\color{black}{ 611007} & \hyperref[subfig:611007]{Nd(As$_{3}$Os)$_{4}$} & 17 & 103 &  0.698 &  0.216 & 204 & 24g,2a,8c & As:2.627 &As:12e &\\
\hline
\color{black}{ 611222} & \hyperref[subfig:611222]{Pr(As$_{3}$Ru)$_{4}$} & 17 & 103 &  0.482 & -0.029 & 204 & 24g,2a,8c & As:2.617 &As:12e &\\
\hline
\color{black}{ 645809} & \hyperref[subfig:645809]{Nd(Sb$_{3}$Ru)$_{4}$} & 17 & 103 &  0.327 & -0.100 & 204 & 24g,2a,8c & Sb:2.890 &Sb:12d &\\
\hline
\color{black}{ 610003} & \hyperref[subfig:610003]{Ce(FeAs$_{3}$)$_{4}$} & 17 & 103 &  0.360 &  0.253 & 204 & 24g,2a,8c & As:2.555 &As:12e &\\
\hline
\color{black}{ 1286} & \hyperref[subfig:1286]{La(FeP$_{3}$)$_{4}$} & 17 & 103 &  0.115 &  0.115 & 204 & 24g,2a,8c &  P:2.288 & P:12e &\\
\hline
\color{black}{ 641615} & \hyperref[subfig:641615]{La(P$_{3}$Os)$_{4}$} & 17 & 103 &  0.422 &  0.079 & 204 & 24g,2a,8c &  P:2.280 & P:12e &\\
\hline
\color{black}{ 645670} & \hyperref[subfig:645670]{Nd(P$_{3}$Os)$_{4}$} & 17 & 103 &  0.018 & -0.325 & 204 & 24g,2a,8c &  P:2.274 & P:12e &\\
\hline
\color{black}{ 155178} & \hyperref[subfig:155178]{Pr(Sb$_{3}$Os)$_{4}$} & 17 & 103 &  0.802 &  0.264 & 204 & 24g,2a,8c & Sb:2.914 &Sb:12d &\\
\hline
\color{black}{ 610776} & \hyperref[subfig:610776]{La(As$_{3}$Os)$_{4}$} & 17 & 103 &  0.784 &  0.506 & 204 & 24g,2a,8c & As:2.631 &As:12e &\\
\hline
\color{black}{ 621737} & \hyperref[subfig:621737]{Ce(Sb$_{3}$Os)$_{4}$} & 17 & 103 &  0.965 &  0.504 & 204 & 24g,2a,8c & Sb:2.958 &Sb:12d &\\
\hline
\color{black}{ 647712} & \hyperref[subfig:647712]{Pr(P$_{3}$Os)$_{4}$} & 17 & 103 &  0.030 & -0.339 & 204 & 24g,2a,8c &  P:2.276 & P:12e &\\
\hline
\color{black}{ 621988} & \hyperref[subfig:621988]{Ce(Sb$_{3}$Ru)$_{4}$} & 17 & 103 &  0.195 & -0.096 & 204 & 24g,2a,8c & Sb:2.909 &Sb:12e &\\
\hline
\color{black}{ 183085} & \hyperref[subfig:183085]{La(Sb$_{3}$Os)$_{4}$} & 17 & 103 &  0.802 &  0.543 & 204 & 24g,2a,8c & Sb:2.911 &Sb:12d &\\
\hline
\color{black}{ 621065} & \hyperref[subfig:621065]{Ce(FeSb$_{3}$)$_{4}$} & 17 & 103 &  0.744 &  0.424 & 204 & 24g,2a,8c & Sb:2.905 &Sb:12d &\\
\hline
\color{black}{ 53490} & \hyperref[subfig:53490]{La(FeSb$_{3}$)$_{4}$} & 17 & 103 &  0.839 &  0.608 & 204 & 24g,2a,8c & Sb:2.932 &Sb:12d &\\
\hline
\color{black}{ 647760} & \hyperref[subfig:647760]{Sm(Sb$_{3}$Os)$_{4}$} & 17 & 103 &  0.758 &  0.182 & 204 & 24g,2a,8c & Sb:2.902 &Sb:12d &\\
\hline
\color{black}{ 280022} & \hyperref[subfig:280022]{Ba$_{5}$Sb$_{4}$} & 18 & 140 &  0.629 &  0.249 &  64 & 8d,8f,4a,16g & Sb:2.886 &Sb:4b  &Ag@4b\\
 & & & & & & & & & &Bg@4b\\
\hline
280143 & \hyperref[subfig:280143]{Tm$_{5}$(ReO$_{6}$)$_{2}$} & 19 & 131 &  0.097 &  0.091 &  12 & 2d,4g,4i,8j &  O:2.665 & O:2a  &Au@2b\\
 & & & & & & & & & &Bu@2b\\
\hline
280002 & \hyperref[subfig:280002]{TiNb$_{3}$O$_{6}$} & 20 & 146 &  0.658 &  0.494 & 148 & 6c,18f &  O:2.670 & O:18f &A1g@3a\\
\hline
10032 & \hyperref[subfig:10032]{AlSiP$_{3}$} & 20 & 88 &  1.264 &  0.274 &  62 & 8d,4c,4a & Si:3.722  P:2.182 &Si:4c   P:4b  &Ag@4b\\
\hline
246145 & \hyperref[subfig:246145]{Bi$_{4}$I} & 20 & 108 &  0.001 & -0.882 &  12 & 4i &  I:4.445 & I:8j  &Ag@2c\&Ag@2b\\
\hline
422527 & \hyperref[subfig:422527]{Sr(GaAs)$_{2}$} & 20 & 104 &  0.252 &  0.252 &  10 & 2m,2n,1d,1c & As:3.888 &As:4o  &Ag@1g\&Ag@1a\\
\hline
262307 & \hyperref[subfig:262307]{Nd$_{2}$SbO$_{2}$} & 20 & 156 &  0.023 & -1.610 &  59 & 2a,4e &  O:2.804 Sb:3.280 & O:4c  Sb:2a  &A@2b\\
 & & & & & & & & & &A2@2b\\
\hline
\color{black}{ 36157} & \hyperref[subfig:36157]{BeSO$_{8}$} & 20 & 112 &  0.000 & -0.133 & 140 & 16k,4c,4d,16l &  S:3.303  O:1.758 & S:4a   O:16j &\\
\hline
200210 & \hyperref[subfig:200210]{Mg$_{3}$Nb$_{6}$O$_{11}$} & 20 & 138 &  0.706 &  0.177 & 164 & 2d,6i,3e,1b &  O:2.846 & O:6i  &A1g@1a\\
\hline
415950 & \hyperref[subfig:415950]{Nb$_{2}$F$_{5}$} & 21 & 171 &  1.091 &  1.041 & 229 & 24h,12e,6b &  F:2.880 & F:24h &A1g@8c\&A2u@8c\\
 & & & & & & & & & &A2g@2a\&A2u@2a\\
\hline
82360 & \hyperref[subfig:82360]{Ba$_{5}$CrN$_{5}$} & 22 & 162 &  0.324 &  0.119 &  12 & 4g,8j,4i &  N:2.821 & N:4g  &Ag@2c\\
\hline
202189 & \hyperref[subfig:202189]{La$_{2}$Mo$_{2}$O$_{7}$} & 22 & 152 &  0.112 & -1.702 &  58 & 2a,4g &  O:2.605 & O:4g  &Ag@2d\&Au@2d\\
 & & & & & & & & & &Ag@2c\&Au@2c\\
\hline
62517 & \hyperref[subfig:62517]{Sr(P$_{3}$Pt$_{2}$)$_{2}$} & 22 & 160 &  0.634 &  0.409 &  15 & 8f,4b,4e,4a &  P:2.173 & P:4c  &Ag@4d\&Ag@4c\\
\hline
25766 & \hyperref[subfig:25766]{Nb$_{3}$Br$_{8}$} & 22 & 178 &  0.070 &  0.070 & 166 & 6c,18h & Br:3.462 &Br:18h &A1g@3b\\
\hline
62519 & \hyperref[subfig:62519]{Ba(As$_{3}$Pt$_{2}$)$_{2}$} & 22 & 160 &  0.329 &  0.259 &  15 & 8f,4b,4e,4a & As:2.411 &As:4d  &Ag@4d\&Ag@4c\\
\hline
62518 & \hyperref[subfig:62518]{Sr(As$_{3}$Pt$_{2}$)$_{2}$} & 22 & 160 &  0.275 &  0.164 &  15 & 8f,4b,4e,4a & As:2.415 &As:4c  &Ag@4d\&Ag@4c\\
\hline
611500 & \hyperref[subfig:611500]{TiAs$_{2}$} & 24 & 112 &  0.000 & -0.612 &  58 & 4g & As:2.576 &As:2b  &Ag@2d\&Ag@2b\\
\hline
\color{black}{ 613517} & \hyperref[subfig:613517]{LuCrB$_{4}$} & 24 & 108 &  0.217 & -0.115 &  55 & 4g,4h &  B:1.586 & B:4h  &\\
\hline
35676 & \hyperref[subfig:35676]{LiGeTe$_{2}$} & 24 & 102 &  0.562 &  0.380 &   2 & 1d,1b,2i & Te:3.860 &Te:2i  &Ag@1g\\
\hline
\color{black}{ 613495} & \hyperref[subfig:613495]{ErCrB$_{4}$} & 24 & 108 &  0.159 & -0.230 &  55 & 4g,4h &  B:1.595 & B:4h  &\\
\hline
62520 & \hyperref[subfig:62520]{BaP$_{3}$Pt$_{2}$} & 24 & 180 &  0.529 &  0.134 &  14 & 2a,4e,2b &  P:2.200 & P:4e  &Ag@2c\\
\hline
\color{black}{ 16171} & \hyperref[subfig:16171]{YCrB$_{4}$} & 24 & 116 &  0.228 & -0.253 &  55 & 4g,4h &  B:1.605 & B:4h  &\\
\hline
39429 & \hyperref[subfig:39429]{TiCl$_{3}$} & 24 & 150 &  0.038 & -0.170 &  12 & 4g,8j,4i & Cl:3.172 &Cl:4e  &Ag@2b\\
 & & & & & & & & & &Bg@2b\\
\hline
\color{black}{ 613514} & \hyperref[subfig:613514]{HoCrB$_{4}$} & 24 & 108 &  0.177 & -0.123 &  55 & 4g,4h &  B:1.600 & B:4h  &\\
\hline
\color{black}{ 20081} & \hyperref[subfig:20081]{YB$_{4}$Mo} & 24 & 116 &  0.150 & -0.480 &  55 & 4g,4h &  B:1.630 & B:4h  &\\
\hline
419780 & \hyperref[subfig:419780]{CoGeTe} & 24 & 152 &  0.171 &  0.097 &  61 & 8c & Te:3.515 &Te:8c  &Ag@4b\\
\hline
645690 & \hyperref[subfig:645690]{NdPS} & 24 & 176 &  0.475 &  0.446 &  62 & 8d,4c &  P:2.309  S:3.455 & P:4b   S:4c  &Ag@4b\\
\hline
260373 & \hyperref[subfig:260373]{GeTeRh} & 24 & 152 &  0.358 &  0.299 &  61 & 8c & Te:3.617 &Te:8c  &Ag@4b\\
\hline
630913 & \hyperref[subfig:630913]{ErPS} & 24 & 160 &  0.319 &  0.308 &  62 & 8d,4c &  P:2.211  S:3.328 & P:4b   S:4c  &Ag@4b\\
\hline
409820 & \hyperref[subfig:409820]{YbNiB$_{4}$} & 24 & 120 &  0.054 & -1.423 &  55 & 4g,4h &  B:1.711 & B:4h  &Ag@2c\&Ag@2b\\
\hline
647960 & \hyperref[subfig:647960]{PrPS} & 24 & 176 &  0.485 &  0.455 &  62 & 8d,4c &  P:2.326  S:3.477 & P:4b   S:4c  &Ag@4b\\
\hline
\color{black}{ 612757} & \hyperref[subfig:612757]{CeCrB$_{4}$} & 24 & 116 &  0.167 &  0.055 &  55 & 4g,4h &  B:1.680 & B:2b  &\\
\hline
\color{black}{ 613559} & \hyperref[subfig:613559]{TbCrB$_{4}$} & 24 & 108 &  0.180 & -0.104 &  55 & 4g,4h &  B:1.606 & B:4h  &\\
\hline
\color{black}{ 658658} & \hyperref[subfig:658658]{DyCrB$_{4}$} & 24 & 108 &  0.154 & -0.173 &  55 & 4g,4h &  B:1.601 & B:4h  &\\
\hline
648073 & \hyperref[subfig:648073]{TmPS} & 24 & 160 &  0.298 &  0.287 &  62 & 8d,4c &  P:2.201  S:3.316 & P:4b   S:4c  &Ag@4b\\
\hline
648080 & \hyperref[subfig:648080]{YPS} & 24 & 176 &  0.365 &  0.356 &  62 & 8d,4c &  P:2.230  S:3.356 & P:4b   S:4c  &Ag@4b\\
\hline
\color{black}{ 300158} & \hyperref[subfig:300158]{KGaSb$_{4}$} & 24 & 128 &  0.296 &  0.296 &  62 & 4c & Sb:2.833 &Sb:4c  &Ag@4a\\
\hline
\color{black}{ 638875} & \hyperref[subfig:638875]{HfSb$_{2}$} & 24 & 112 &  0.016 & -0.659 &  58 & 4g & Sb:2.893 &Sb:2a  &Ag@2c\&Ag@2a\\
\hline
\color{black}{ 418567} & \hyperref[subfig:418567]{Y$_{4}$InIr} & 24 & 224 &  0.000 & -0.140 & 216 & 24g,24f,16e & &&A1@4c\&A1@4b\\
 & & & & & & & & & &A1@4c\&T1@4b\\
 & & & & & & & & & &T1@4c\&A1@4b\\
 & & & & & & & & & &T1@4c\&T1@4b\\
\hline
\color{black}{ 42880} & \hyperref[subfig:42880]{ZrBi$_{2}$} & 24 & 176 &  0.001 & -0.538 &  58 & 4g & &&Ag@2c\&Ag@2a\\
\hline
\color{black}{ 418270} & \hyperref[subfig:418270]{Ho$_{4}$InIr} & 24 & 192 &  0.000 & -0.157 & 216 & 24g,24f,16e & &&A1@4d\&A1@4b\\
 & & & & & & & & & &A1@4d\&T1@4b\\
 & & & & & & & & & &T1@4d\&A1@4b\\
 & & & & & & & & & &T1@4d\&T1@4b\\
\hline
\color{black}{ 418265} & \hyperref[subfig:418265]{Er$_{4}$InIr} & 24 & 192 &  0.000 & -0.139 & 216 & 24g,24f,16e & &&A1@4d\&A1@4b\\
 & & & & & & & & & &A1@4d\&T1@4b\\
 & & & & & & & & & &T1@4d\&A1@4b\\
 & & & & & & & & & &T1@4d\&T1@4b\\
\hline
\color{black}{ 66779} & \hyperref[subfig:66779]{ZrSb$_{2}$} & 24 & 176 &  0.021 & -0.661 &  58 & 4g & Sb:2.879 &Sb:2b  &Ag@2d\&Ag@2b\\
\hline
648052 & \hyperref[subfig:648052]{SmPS} & 24 & 176 &  0.444 &  0.417 &  62 & 8d,4c &  P:2.281  S:3.419 & P:4b   S:4c  &Ag@4b\\
\hline
\color{black}{ 616683} & \hyperref[subfig:616683]{HfBi$_{2}$} & 24 & 112 &  0.001 & -0.747 &  58 & 4g & &&Ag@2c\&Ag@2a\\
\hline
404707 & \hyperref[subfig:404707]{Ba$_{2}$LiSi$_{3}$} & 24 & 132 &  0.106 &  0.102 &  70 & 32h,16g,16f & Si:2.382 &Si:32h &A@8b\\
 & & & & & & & & & &B3@8b\\
 & & & & & & & & & &A@8a\\
 & & & & & & & & & &B3@8a\\
\hline
\color{black}{ 417519} & \hyperref[subfig:417519]{Tm$_{4}$InRh} & 24 & 192 &  0.018 & -0.114 & 216 & 24g,24f,16e & &&A1@4c\&A1@4a\\
 & & & & & & & & & &A1@4c\&T1@4a\\
 & & & & & & & & & &T1@4c\&A1@4a\\
 & & & & & & & & & &T1@4c\&T1@4a\\
\hline
\color{black}{ 417518} & \hyperref[subfig:417518]{Tb$_{4}$InRh} & 24 & 192 &  0.000 & -0.222 & 216 & 24g,24f,16e & &&A1@4c\&A1@4b\\
 & & & & & & & & & &A1@4c\&T1@4b\\
 & & & & & & & & & &T1@4c\&A1@4b\\
 & & & & & & & & & &T1@4c\&T1@4b\\
\hline
\color{black}{ 404705} & \hyperref[subfig:404705]{Ba$_{2}$LiGe$_{3}$} & 24 & 132 &  0.151 &  0.096 &  70 & 32h,16g,16f & &&A@8b\\
 & & & & & & & & & &B3@8b\\
 & & & & & & & & & &A@8a\\
 & & & & & & & & & &B3@8a\\
\hline
\color{black}{ 417517} & \hyperref[subfig:417517]{Ho$_{4}$InRh} & 24 & 192 &  0.002 & -0.200 & 216 & 24g,24f,16e & &&A1@4c\&A1@4b\\
 & & & & & & & & & &A1@4c\&T1@4b\\
 & & & & & & & & & &T1@4c\&A1@4b\\
 & & & & & & & & & &T1@4c\&T1@4b\\
\hline
409295 & \hyperref[subfig:409295]{Sr$_{2}$LiSi$_{3}$} & 24 & 132 &  0.020 & -0.100 &  70 & 32h,16g,16f & Si:2.377 &Si:16e &A@8b\\
 & & & & & & & & & &B3@8b\\
 & & & & & & & & & &A@8a\\
 & & & & & & & & & &B3@8a\\
\hline
\color{black}{ 300157} & \hyperref[subfig:300157]{KAlSb$_{4}$} & 24 & 128 &  0.246 &  0.246 &  62 & 4c & Sb:2.828 &Sb:4c  &Ag@4a\\
\hline
89380 & \hyperref[subfig:89380]{FeS} & 24 & 168 &  0.020 &  0.015 &  14 & 4e &  S:2.910 & S:4e  &Ag@2d\&Ag@2a\\
\hline
410520 & \hyperref[subfig:410520]{Ba$_{2}$Si$_{3}$Ag} & 24 & 172 &  0.092 &  0.010 &  70 & 32h,16g,16f & Si:2.377 &Si:32h &A@8b\\
 & & & & & & & & & &B3@8b\\
 & & & & & & & & & &A@8a\\
 & & & & & & & & & &B3@8a\\
\hline
\color{black}{ 262063} & \hyperref[subfig:262063]{KTl} & 24 & 144 &  0.100 &  0.013 &  64 & 8d,8f,8e,16g & &&Ag@4b\&Ag@4b\\
 & & & & & & & & & &Ag@4b\&Bg@4b\\
 & & & & & & & & & &Bg@4b\&Bg@4b\\
\hline
648063 & \hyperref[subfig:648063]{TbPS} & 24 & 160 &  0.385 &  0.375 &  62 & 8d,4c &  P:2.242  S:3.370 & P:4b   S:4c  &Ag@4b\\
\hline
639545 & \hyperref[subfig:639545]{HoPS} & 24 & 160 &  0.347 &  0.336 &  62 & 8d,4c &  P:2.221  S:3.342 & P:4b   S:4c  &Ag@4b\\
\hline
641637 & \hyperref[subfig:641637]{LaPS} & 24 & 176 &  0.464 &  0.455 &  62 & 8d,4c &  P:2.373  S:3.539 & P:4b   S:4c  &Ag@4b\\
\hline
\color{black}{ 280592} & \hyperref[subfig:280592]{Ba$_{3}$Sb$_{2}$O} & 24 & 184 &  0.468 &  0.372 &  55 & 4g,4h & Sb:2.837  O:6.336 &Sb:2d   O:4g  &Ag@2d\&Ag@2b\\
\hline
\color{black}{ 417514} & \hyperref[subfig:417514]{Dy$_{4}$InRh} & 24 & 192 &  0.003 & -0.206 & 216 & 24g,24f,16e & &&A1@4d\&A1@4b\\
 & & & & & & & & & &A1@4d\&T1@4b\\
 & & & & & & & & & &T1@4d\&A1@4b\\
 & & & & & & & & & &T1@4d\&T1@4b\\
\hline
630062 & \hyperref[subfig:630062]{DyPS} & 24 & 160 &  0.366 &  0.356 &  62 & 8d,4c &  P:2.232  S:3.356 & P:4b   S:4c  &Ag@4b\\
\hline
\color{black}{ 417515} & \hyperref[subfig:417515]{Er$_{4}$InRh} & 24 & 192 &  0.002 & -0.162 & 216 & 24g,24f,16e & &&A1@4c\&A1@4b\\
 & & & & & & & & & &A1@4c\&T1@4b\\
 & & & & & & & & & &T1@4c\&A1@4b\\
 & & & & & & & & & &T1@4c\&T1@4b\\
\hline
413194 & \hyperref[subfig:413194]{SiSbPt} & 24 & 152 &  0.413 &  0.253 &  61 & 8c & Sb:3.585 Si:3.432 &Sb:8c  Si:8c  &Ag@4a\\
\hline
\color{black}{ 186915} & \hyperref[subfig:186915]{Yb(Al$_{5}$Ru)$_{2}$} & 26 & 108 &  0.003 & -0.358 &  63 & 8d,8f,8e,4c,8g & &&Ag@4b\&Ag@4a\\
 & & & & & & & & & &Ag@4b\&Bg@4a\\
 & & & & & & & & & &Bg@4b\&Ag@4a\\
 & & & & & & & & & &Bg@4b\&Bg@4a\\
\hline
29261 & \hyperref[subfig:29261]{Ba$_{3}$(Si$_{2}$P$_{3}$)$_{2}$} & 26 & 152 &  0.413 &  0.413 &  11 & 4f,2e & Si:2.383  P:3.666 &Si:2c   P:2e  &Ag@2c\\
\hline
\color{black}{ 238040} & \hyperref[subfig:238040]{Yb(Al$_{5}$Os)$_{2}$} & 26 & 108 &  0.008 & -0.304 &  63 & 8d,8f,8e,4c,8g & &&Ag@4b\&Ag@4a\\
 & & & & & & & & & &Ag@4b\&Bg@4a\\
 & & & & & & & & & &Bg@4b\&Ag@4a\\
 & & & & & & & & & &Bg@4b\&Bg@4a\\
\hline
\color{black}{ 151140} & \hyperref[subfig:151140]{Yb(Al$_{5}$Fe)$_{2}$} & 26 & 108 &  0.002 & -0.207 &  63 & 8d,8f,8e,4c,8g & &&Ag@4b\&Ag@4a\\
 & & & & & & & & & &Ag@4b\&Bg@4a\\
 & & & & & & & & & &Bg@4b\&Ag@4a\\
 & & & & & & & & & &Bg@4b\&Bg@4a\\
\hline
165596 & \hyperref[subfig:165596]{CuAgPO$_{4}$} & 28 & 204 &  0.092 &  0.092 &  14 & 4e &  P:3.736  O:2.437 & P:2d   O:4e  &Au@2b\\
\hline
411801 & \hyperref[subfig:411801]{La$_{3}$PI$_{3}$} & 28 & 236 &  0.013 & -0.361 & 214 & 24g,8a &  I:3.850  P:4.394 & I:12d  P:12c &A@12d\\
 & & & & & & & & & &B1@12d\\
 & & & & & & & & & &A@12c\\
 & & & & & & & & & &B1@12c\\
\hline
26565 & \hyperref[subfig:26565]{Cs$_{3}$Zr$_{2}$I$_{9}$} & 28 & 228 &  0.517 &  0.326 & 194 & 4f,12k,6h,2b &  I:3.998 & I:24l &A1'@2d\\
 & & & & & & & & & &A2'@2d\\
 & & & & & & & & & &E''@2d\\
\hline
\color{black}{ 48168} & \hyperref[subfig:48168]{Na$_{7}$Al$_{2}$Sb$_{5}$} & 28 & 76 &  0.506 &  0.316 &  11 & 4f,2e & Sb:2.900 &Sb:2d  &Ag@2d\\
\hline
411803 & \hyperref[subfig:411803]{La$_{3}$AsI$_{3}$} & 28 & 236 &  0.019 & -0.343 & 214 & 24g,8b &  I:4.063 As:4.431 & I:12c As:12d &A@12d\\
 & & & & & & & & & &A@12c\\
\hline
\color{black}{ 413701} & \hyperref[subfig:413701]{Sr$_{11}$(CdSb$_{2}$)$_{6}$} & 29 & 242 &  0.285 &  0.285 &  12 & 2a,4i & Sb:2.814 &Sb:2d  &Ag@2d\\
\hline
\color{black}{ 418886} & \hyperref[subfig:418886]{Ba$_{11}$(CdSb$_{2}$)$_{6}$} & 29 & 242 &  0.114 &  0.114 &  12 & 2a,4i & Sb:2.812 &Sb:2d  &Ag@2d\\
\hline
\color{black}{ 107097} & \hyperref[subfig:107097]{Nb$_{6}$Fe$_{16}$Si$_{7}$} & 29 & 222 &  0.011 & -0.029 & 225 & 24e,24d,32f,4b & Si:4.007 &Si:96k &\\
\hline
\color{black}{ 107098} & \hyperref[subfig:107098]{Ta$_{6}$Fe$_{16}$Si$_{7}$} & 29 & 186 &  0.005 & -0.054 & 225 & 24e,24d,32f,4b & Si:3.992 &Si:96k &\\
\hline
\color{black}{ 643287} & \hyperref[subfig:643287]{Mn$_{2}$P$_{12}$W} & 30 & 160 &  0.323 &  0.014 &  15 & 8f,4e &  P:2.192 & P:8f  &\\
\hline
427778 & \hyperref[subfig:427778]{Ba$_{4}$Li$_{2}$(CdAs$_{2}$)$_{3}$} & 30 & 216 &  0.367 &  0.325 &  63 & 8f,4c & As:2.510 &As:4b  &Ag@4b\\
\hline
\color{black}{ 68107} & \hyperref[subfig:68107]{Mn$_{2}$MoP$_{12}$} & 30 & 160 &  0.322 &  0.111 &  15 & 8f,4e &  P:2.187 & P:4d  &\\
\hline
280615 & \hyperref[subfig:280615]{Sb$_{2}$MoSe} & 32 & 176 &  0.209 & -0.334 &  14 & 4e & Sb:2.854 Se:3.246 &Sb:4e  Se:4e  &Ag@2d\&Ag@2b\\
\hline
\color{black}{ 108870} & \hyperref[subfig:108870]{Ta$_{3}$Ge} & 32 & 152 &  0.000 & -0.263 &  86 & 8g & &&\\
\hline
\color{black}{ 165617} & \hyperref[subfig:165617]{SrSn$_{3}$Sb$_{4}$} & 32 & 168 &  0.097 & -0.308 &  62 & 4c & Sb:2.920 &Sb:4a  &Ag@4a\\
\hline
380397 & \hyperref[subfig:380397]{RbNb$_{4}$Br$_{11}$} & 32 & 260 &  0.276 &  0.223 &  51 & 2f,4j,8l,4k,2e,4h,4i & Br:3.435 &Br:8l  &Ag@2c\\
 & & & & & & & & & &Bg@2c\\
\hline
\color{black}{ 409434} & \hyperref[subfig:409434]{NaSn} & 32 & 80 &  0.414 &  0.363 & 142 & 32g,16e,16f & &&A@8b\&B1@8b\\
 & & & & & & & & & &A@8a\&B@8a\\
\hline
\color{black}{ 105156} & \hyperref[subfig:105156]{NaPb} & 32 & 80 &  0.010 & -0.050 & 142 & 32g,16e,16f & &&A@8b\&B1@8b\\
 & & & & & & & & & &A@8a\&B@8a\\
\hline
88202 & \hyperref[subfig:88202]{TlCu$_{5}$Se$_{3}$} & 36 & 304 &  0.283 &  0.150 & 136 & 4f,8i & Se:3.661 &Se:2b  &Ag@2b\&B3u@2b\\
 & & & & & & & & & &Au@2b\&B3g@2b\\
 & & & & & & & & & &Ag@2a\&B2u@2a\\
 & & & & & & & & & &Au@2a\&B2g@2a\\
\hline
\color{black}{ 79796} & \hyperref[subfig:79796]{Ta$_{4}$FeTe$_{4}$} & 36 & 208 &  0.001 & -0.403 &  55 & 4e,4g,4h & Te:3.800 &Te:8i  &\\
\hline
\color{black}{ 404695} & \hyperref[subfig:404695]{K$_{6}$Na$_{14}$MgTl$_{18}$} & 39 & 124 &  0.125 &  0.018 & 200 & 8i,1a,6h,6f,6g,12j & &&Ag@1b\&1Au@1a\\
\hline
\color{black}{ 236348} & \hyperref[subfig:236348]{K$_{6}$Na$_{14}$Tl$_{18}$Zn} & 39 & 134 &  0.151 & -0.047 & 200 & 8i,1a,6h,6f,6g,12j & &&Ag@1b\&1Au@1a\\
\hline
\color{black}{ 637743} & \hyperref[subfig:637743]{Ge$_{3}$Ru$_{2}$} & 40 & 224 &  0.396 &  0.394 &  60 & 8d,4c & &&Ag@4b\&Ag@4a\\
\hline
2344 & \hyperref[subfig:2344]{Si$_{3}$Ru$_{2}$} & 40 & 224 &  0.494 &  0.494 &  60 & 8d,4c & Si:2.659 &Si:8d  &Ag@4b\&Ag@4a\\
\hline
\color{black}{ 413518} & \hyperref[subfig:413518]{Ba$_{11}$Sb$_{10}$} & 42 & 320 &  0.083 & -0.305 &  71 & 4j,8l,8m,16o,4f,8n,4h,4i & Sb:2.776 &Sb:4g  &\\
\hline
\color{black}{ 82529} & \hyperref[subfig:82529]{Ba$_{2}$(SnSb$_{2}$)$_{3}$} & 44 & 248 &  0.058 & -0.025 &  62 & 4c & Sb:2.902 &Sb:4a  &Ag@4a\\
\hline
\color{black}{ 39873} & \hyperref[subfig:39873]{YB$_{7}$Mo$_{3}$} & 44 & 200 &  0.016 & -0.586 &  62 & 4c &  B:1.740 & B:4c  &Ag@4a\\
\hline
402661 & \hyperref[subfig:402661]{Y$_{4}$BBr$_{6}$} & 44 & 356 &  0.002 & -0.274 &  15 & 8f & Br:3.730  B:3.949 &Br:4d   B:4e  &A@4e\\
\hline
410997 & \hyperref[subfig:410997]{Tb$_{4}$BBr$_{6}$} & 44 & 324 &  0.009 & -0.309 &  15 & 8f & Br:3.751  B:3.943 &Br:4d   B:4b  &A@4e\\
\hline
79976 & \hyperref[subfig:79976]{BaNb$_{8}$O$_{14}$} & 46 & 364 &  0.440 &  0.323 &  55 & 2d,2a,4g,8i,4h,2c &  O:2.678 & O:8i  &Ag@2b\\
\hline
202674 & \hyperref[subfig:202674]{SrNb$_{8}$O$_{14}$} & 46 & 364 &  0.239 &  0.171 &  55 & 2d,2a,4g,8i,4h,2c &  O:2.614 & O:8i  &Ag@2b\\
\hline
\color{black}{ 165180} & \hyperref[subfig:165180]{K(NaIn$_{3}$)$_{3}$} & 52 & 156 &  0.072 &  0.009 &  64 & 8f,8e,16g & &&Au@4b\\
\hline
72021 & \hyperref[subfig:72021]{Nb$_{3}$Se$_{12}$I} & 64 & 448 &  0.105 &  0.104 & 128 & 8f,16i,8h,4e,4d &  I:4.953 Se:2.358 & I:2a  Se:8h  &Ag@4c\\
 & & & & & & & & & &Bg@4c\\
\hline
\color{black}{ 103709} & \hyperref[subfig:103709]{K$_{3}$Ga$_{13}$} & 64 & 264 &  0.140 & -0.045 &  63 & 8f,4c,8g,16h & &&\\
\hline
\color{black}{ 165613} & \hyperref[subfig:165613]{Na$_{5}$Sn$_{13}$} & 144 & 456 &  0.000 & -0.283 &  63 & 8f,4c,8g,16h & &&Ag@4b\\
\hline
\end{longtable}
\begin{figure}[htp]
 \centering
\subfigure[GdO SG216 NoA=2 NoE=15]{
\label{subfig:24981}
\includegraphics[scale=0.32,angle=270]{mater-band/24981}
}
\subfigure[MnP SG216 NoA=2 NoE=12]{
\label{subfig:191788}
\includegraphics[scale=0.32,angle=270]{mater-band/191788}
}
\subfigure[MnN SG216 NoA=2 NoE=12]{
\label{subfig:236788}
\includegraphics[scale=0.32,angle=270]{mater-band/236788}
}
\subfigure[MnSn SG216 NoA=2 NoE=11]{
\label{subfig:191171}
\includegraphics[scale=0.32,angle=270]{mater-band/191171}
}
\subfigure[HfN SG216 NoA=2 NoE=9]{
\label{subfig:167875}
\includegraphics[scale=0.32,angle=270]{mater-band/167875}
}
\subfigure[TaN SG216 NoA=2 NoE=10]{
\label{subfig:167876}
\includegraphics[scale=0.32,angle=270]{mater-band/167876}
}
\subfigure[SiP SG216 NoA=2 NoE=9]{
\label{subfig:30334}
\includegraphics[scale=0.32,angle=270]{mater-band/30334}
}
\subfigure[TcN SG216 NoA=2 NoE=12]{
\label{subfig:167870}
\includegraphics[scale=0.32,angle=270]{mater-band/167870}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[MoP SG216 NoA=2 NoE=11]{
\label{subfig:186876}
\includegraphics[scale=0.32,angle=270]{mater-band/186876}
}
\subfigure[IrN SG216 NoA=2 NoE=14]{
\label{subfig:186243}
\includegraphics[scale=0.32,angle=270]{mater-band/186243}
}
\subfigure[RhN SG216 NoA=2 NoE=14]{
\label{subfig:183192}
\includegraphics[scale=0.32,angle=270]{mater-band/183192}
}
\subfigure[RuN SG216 NoA=2 NoE=13]{
\label{subfig:183190}
\includegraphics[scale=0.32,angle=270]{mater-band/183190}
}
\subfigure[Cu SG12 NoA=2 NoE=22]{
\label{subfig:150682}
\includegraphics[scale=0.32,angle=270]{mater-band/150682}
}
\subfigure[NbN SG216 NoA=2 NoE=16]{
\label{subfig:183184}
\includegraphics[scale=0.32,angle=270]{mater-band/183184}
}
\subfigure[MoN SG216 NoA=2 NoE=11]{
\label{subfig:187182}
\includegraphics[scale=0.32,angle=270]{mater-band/187182}
}
\subfigure[FeN SG216 NoA=2 NoE=13]{
\label{subfig:41258}
\includegraphics[scale=0.32,angle=270]{mater-band/41258}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[ZrN SG216 NoA=2 NoE=17]{
\label{subfig:183182}
\includegraphics[scale=0.32,angle=270]{mater-band/183182}
}
\subfigure[CrN SG216 NoA=2 NoE=11]{
\label{subfig:181079}
\includegraphics[scale=0.32,angle=270]{mater-band/181079}
}
\subfigure[OsN SG216 NoA=2 NoE=13]{
\label{subfig:167879}
\includegraphics[scale=0.32,angle=270]{mater-band/167879}
}
\subfigure[Ca$_{2}$N SG166 NoA=3 NoE=25]{
\label{subfig:22231}
\includegraphics[scale=0.32,angle=270]{mater-band/22231}
}
\subfigure[NbS$_{2}$ SG187 NoA=3 NoE=23]{
\label{subfig:67443}
\includegraphics[scale=0.32,angle=270]{mater-band/67443}
}
\subfigure[KO$_{2}$ SG139 NoA=3 NoE=21]{
\label{subfig:38245}
\includegraphics[scale=0.32,angle=270]{mater-band/38245}
}
\subfigure[HfN$_{2}$ SG187 NoA=3 NoE=14]{
\label{subfig:290427}
\includegraphics[scale=0.32,angle=270]{mater-band/290427}
}
\subfigure[HgO$_{2}$ SG12 NoA=3 NoE=24]{
\label{subfig:48214}
\includegraphics[scale=0.32,angle=270]{mater-band/48214}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[TaN$_{2}$ SG187 NoA=3 NoE=15]{
\label{subfig:290430}
\includegraphics[scale=0.32,angle=270]{mater-band/290430}
}
\subfigure[MnNiSb SG216 NoA=3 NoE=22]{
\label{subfig:54255}
\includegraphics[scale=0.32,angle=270]{mater-band/54255}
}
\subfigure[CrSe$_{2}$ SG12 NoA=3 NoE=18]{
\label{subfig:251718}
\includegraphics[scale=0.32,angle=270]{mater-band/251718}
}
\subfigure[Sr$_{2}$N SG166 NoA=3 NoE=25]{
\label{subfig:414330}
\includegraphics[scale=0.32,angle=270]{mater-band/414330}
}
\subfigure[RbO$_{2}$ SG139 NoA=3 NoE=21]{
\label{subfig:647338}
\includegraphics[scale=0.32,angle=270]{mater-band/647338}
}
\subfigure[Al$_{2}$Os SG139 NoA=3 NoE=14]{
\label{subfig:58108}
\includegraphics[scale=0.32,angle=270]{mater-band/58108}
}
\subfigure[MnSnAu SG216 NoA=3 NoE=22]{
\label{subfig:54465}
\includegraphics[scale=0.32,angle=270]{mater-band/54465}
}
\subfigure[LiFeP SG107 NoA=3 NoE=14]{
\label{subfig:187135}
\includegraphics[scale=0.32,angle=270]{mater-band/187135}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Mg$_{3}$In SG221 NoA=4 NoE=9]{
\label{subfig:51975}
\includegraphics[scale=0.32,angle=270]{mater-band/51975}
}
\subfigure[TiAlFe$_{2}$ SG225 NoA=4 NoE=23]{
\label{subfig:57827}
\includegraphics[scale=0.32,angle=270]{mater-band/57827}
}
\subfigure[LiAl SG227 NoA=4 NoE=8]{
\label{subfig:240110}
\includegraphics[scale=0.32,angle=270]{mater-band/240110}
}
\subfigure[AlVFe$_{2}$ SG225 NoA=4 NoE=24]{
\label{subfig:57832}
\includegraphics[scale=0.32,angle=270]{mater-band/57832}
}
\subfigure[ZrCd SG129 NoA=4 NoE=48]{
\label{subfig:620612}
\includegraphics[scale=0.32,angle=270]{mater-band/620612}
}
\subfigure[TiFe$_{2}$Sn SG225 NoA=4 NoE=24]{
\label{subfig:633766}
\includegraphics[scale=0.32,angle=270]{mater-band/633766}
}
\subfigure[FeSiRu$_{2}$ SG225 NoA=4 NoE=28]{
\label{subfig:633246}
\includegraphics[scale=0.32,angle=270]{mater-band/633246}
}
\subfigure[ZrCl SG164 NoA=4 NoE=38]{
\label{subfig:35701}
\includegraphics[scale=0.32,angle=270]{mater-band/35701}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[VGaFe$_{2}$ SG225 NoA=4 NoE=24]{
\label{subfig:631850}
\includegraphics[scale=0.32,angle=270]{mater-band/631850}
}
\subfigure[HfBe SG63 NoA=4 NoE=12]{
\label{subfig:616286}
\includegraphics[scale=0.32,angle=270]{mater-band/616286}
}
\subfigure[SrMgIn$_{3}$ SG119 NoA=5 NoE=21]{
\label{subfig:249592}
\includegraphics[scale=0.32,angle=270]{mater-band/249592}
}
\subfigure[Ge$_{2}$Os SG12 NoA=6 NoE=32]{
\label{subfig:43690}
\includegraphics[scale=0.32,angle=270]{mater-band/43690}
}
\subfigure[YMgCu$_{4}$ SG216 NoA=6 NoE=57]{
\label{subfig:163696}
\includegraphics[scale=0.32,angle=270]{mater-band/163696}
}
\subfigure[Al$_{2}$Ru SG70 NoA=6 NoE=28]{
\label{subfig:58156}
\includegraphics[scale=0.32,angle=270]{mater-band/58156}
}
\subfigure[CaInCu$_{4}$ SG216 NoA=6 NoE=57]{
\label{subfig:658914}
\includegraphics[scale=0.32,angle=270]{mater-band/658914}
}
\subfigure[NdMgCu$_{4}$ SG216 NoA=6 NoE=57]{
\label{subfig:194977}
\includegraphics[scale=0.32,angle=270]{mater-band/194977}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Be$_{5}$Pd SG216 NoA=6 NoE=20]{
\label{subfig:616387}
\includegraphics[scale=0.32,angle=270]{mater-band/616387}
}
\subfigure[ScInCu$_{4}$ SG216 NoA=6 NoE=50]{
\label{subfig:416528}
\includegraphics[scale=0.32,angle=270]{mater-band/416528}
}
\subfigure[HfGaAu SG187 NoA=6 NoE=36]{
\label{subfig:156265}
\includegraphics[scale=0.32,angle=270]{mater-band/156265}
}
\subfigure[ZrGaAu SG187 NoA=6 NoE=52]{
\label{subfig:156264}
\includegraphics[scale=0.32,angle=270]{mater-band/156264}
}
\subfigure[Be$_{5}$Pt SG216 NoA=6 NoE=20]{
\label{subfig:616395}
\includegraphics[scale=0.32,angle=270]{mater-band/616395}
}
\subfigure[FeSe$_{2}$ SG58 NoA=6 NoE=40]{
\label{subfig:44751}
\includegraphics[scale=0.32,angle=270]{mater-band/44751}
}
\subfigure[MgCu$_{4}$Sn SG216 NoA=6 NoE=50]{
\label{subfig:103055}
\includegraphics[scale=0.32,angle=270]{mater-band/103055}
}
\subfigure[FeSb$_{2}$ SG58 NoA=6 NoE=36]{
\label{subfig:186627}
\includegraphics[scale=0.32,angle=270]{mater-band/186627}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[YInCu$_{4}$ SG216 NoA=6 NoE=58]{
\label{subfig:628179}
\includegraphics[scale=0.32,angle=270]{mater-band/628179}
}
\subfigure[KSb$_{2}$ SG12 NoA=6 NoE=38]{
\label{subfig:80945}
\includegraphics[scale=0.32,angle=270]{mater-band/80945}
}
\subfigure[Ga$_{2}$Ru SG70 NoA=6 NoE=28]{
\label{subfig:635228}
\includegraphics[scale=0.32,angle=270]{mater-band/635228}
}
\subfigure[ZrCu$_{4}$Ag SG216 NoA=6 NoE=67]{
\label{subfig:196260}
\includegraphics[scale=0.32,angle=270]{mater-band/196260}
}
\subfigure[P$_{2}$W SG12 NoA=6 NoE=32]{
\label{subfig:648286}
\includegraphics[scale=0.32,angle=270]{mater-band/648286}
}
\subfigure[Sb$_{2}$Os SG58 NoA=6 NoE=36]{
\label{subfig:238254}
\includegraphics[scale=0.32,angle=270]{mater-band/238254}
}
\subfigure[ScSiAu SG187 NoA=6 NoE=36]{
\label{subfig:71998}
\includegraphics[scale=0.32,angle=270]{mater-band/71998}
}
\subfigure[SrAl$_{2}$ SG74 NoA=6 NoE=32]{
\label{subfig:609407}
\includegraphics[scale=0.32,angle=270]{mater-band/609407}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[RbSb$_{2}$ SG12 NoA=6 NoE=38]{
\label{subfig:419402}
\includegraphics[scale=0.32,angle=270]{mater-band/419402}
}
\subfigure[Si$_{2}$Os SG12 NoA=6 NoE=32]{
\label{subfig:647776}
\includegraphics[scale=0.32,angle=270]{mater-band/647776}
}
\subfigure[YbNi$_{4}$Au SG216 NoA=6 NoE=59]{
\label{subfig:612234}
\includegraphics[scale=0.32,angle=270]{mater-band/612234}
}
\subfigure[Be$_{5}$Co SG216 NoA=6 NoE=19]{
\label{subfig:616209}
\includegraphics[scale=0.32,angle=270]{mater-band/616209}
}
\subfigure[ErCdCu$_{4}$ SG216 NoA=6 NoE=65]{
\label{subfig:415196}
\includegraphics[scale=0.32,angle=270]{mater-band/415196}
}
\subfigure[HoCdCu$_{4}$ SG216 NoA=6 NoE=65]{
\label{subfig:415195}
\includegraphics[scale=0.32,angle=270]{mater-band/415195}
}
\subfigure[Sb$_{2}$Ru SG58 NoA=6 NoE=36]{
\label{subfig:43652}
\includegraphics[scale=0.32,angle=270]{mater-band/43652}
}
\subfigure[As$_{2}$W SG12 NoA=6 NoE=32]{
\label{subfig:611576}
\includegraphics[scale=0.32,angle=270]{mater-band/611576}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[CrAs$_{2}$ SG12 NoA=6 NoE=32]{
\label{subfig:43898}
\includegraphics[scale=0.32,angle=270]{mater-band/43898}
}
\subfigure[As$_{2}$Ru SG58 NoA=6 NoE=36]{
\label{subfig:42578}
\includegraphics[scale=0.32,angle=270]{mater-band/42578}
}
\subfigure[Na$_{2}$Cl SG65 NoA=6 NoE=18]{
\label{subfig:190546}
\includegraphics[scale=0.32,angle=270]{mater-band/190546}
}
\subfigure[CrP$_{2}$ SG12 NoA=6 NoE=32]{
\label{subfig:2526}
\includegraphics[scale=0.32,angle=270]{mater-band/2526}
}
\subfigure[LiYGa$_{4}$ SG187 NoA=6 NoE=24]{
\label{subfig:98666}
\includegraphics[scale=0.32,angle=270]{mater-band/98666}
}
\subfigure[MgInCu$_{4}$ SG216 NoA=6 NoE=49]{
\label{subfig:628018}
\includegraphics[scale=0.32,angle=270]{mater-band/628018}
}
\subfigure[PbSe$_{2}$ SG140 NoA=6 NoE=32]{
\label{subfig:174577}
\includegraphics[scale=0.32,angle=270]{mater-band/174577}
}
\subfigure[ZrCu$_{5}$ SG216 NoA=6 NoE=67]{
\label{subfig:191404}
\includegraphics[scale=0.32,angle=270]{mater-band/191404}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[ReN$_{2}$ SG12 NoA=6 NoE=34]{
\label{subfig:187441}
\includegraphics[scale=0.32,angle=270]{mater-band/187441}
}
\subfigure[BaTe$_{2}$ SG140 NoA=6 NoE=44]{
\label{subfig:75555}
\includegraphics[scale=0.32,angle=270]{mater-band/75555}
}
\subfigure[Te$_{2}$Ru SG58 NoA=6 NoE=40]{
\label{subfig:106001}
\includegraphics[scale=0.32,angle=270]{mater-band/106001}
}
\subfigure[MoAs$_{2}$ SG5 NoA=6 NoE=32]{
\label{subfig:16820}
\includegraphics[scale=0.32,angle=270]{mater-band/16820}
}
\subfigure[FeP$_{2}$ SG58 NoA=6 NoE=36]{
\label{subfig:633072}
\includegraphics[scale=0.32,angle=270]{mater-band/633072}
}
\subfigure[YbInCu$_{4}$ SG216 NoA=6 NoE=55]{
\label{subfig:628189}
\includegraphics[scale=0.32,angle=270]{mater-band/628189}
}
\subfigure[FeTe$_{2}$ SG58 NoA=6 NoE=40]{
\label{subfig:633866}
\includegraphics[scale=0.32,angle=270]{mater-band/633866}
}
\subfigure[YGaI SG164 NoA=6 NoE=42]{
\label{subfig:417149}
\includegraphics[scale=0.32,angle=270]{mater-band/417149}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[FeAs$_{2}$ SG58 NoA=6 NoE=36]{
\label{subfig:65168}
\includegraphics[scale=0.32,angle=270]{mater-band/65168}
}
\subfigure[TbInCu$_{4}$ SG216 NoA=6 NoE=56]{
\label{subfig:152560}
\includegraphics[scale=0.32,angle=270]{mater-band/152560}
}
\subfigure[V(MoS$_{2}$)$_{2}$ SG12 NoA=7 NoE=41]{
\label{subfig:201787}
\includegraphics[scale=0.32,angle=270]{mater-band/201787}
}
\subfigure[KB$_{6}$ SG221 NoA=7 NoE=27]{
\label{subfig:98990}
\includegraphics[scale=0.32,angle=270]{mater-band/98990}
}
\subfigure[Rb$_{2}$Te$_{5}$ SG12 NoA=7 NoE=48]{
\label{subfig:30734}
\includegraphics[scale=0.32,angle=270]{mater-band/30734}
}
\subfigure[SiB$_{6}$ SG221 NoA=7 NoE=22]{
\label{subfig:20240}
\includegraphics[scale=0.32,angle=270]{mater-band/20240}
}
\subfigure[NaCl$_{7}$ SG200 NoA=8 NoE=50]{
\label{subfig:190537}
\includegraphics[scale=0.32,angle=270]{mater-band/190537}
}
\subfigure[SiRh SG14 NoA=8 NoE=52]{
\label{subfig:79235}
\includegraphics[scale=0.32,angle=270]{mater-band/79235}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Ge SG148 NoA=8 NoE=32]{
\label{subfig:245961}
\includegraphics[scale=0.32,angle=270]{mater-band/245961}
}
\subfigure[InP$_{3}$ SG166 NoA=8 NoE=36]{
\label{subfig:37073}
\includegraphics[scale=0.32,angle=270]{mater-band/37073}
}
\subfigure[LaSi SG63 NoA=8 NoE=60]{
\label{subfig:408030}
\includegraphics[scale=0.32,angle=270]{mater-band/408030}
}
\subfigure[TaInS$_{2}$ SG194 NoA=8 NoE=40]{
\label{subfig:640379}
\includegraphics[scale=0.32,angle=270]{mater-band/640379}
}
\subfigure[Te$_{2}$AuI SG51 NoA=8 NoE=60]{
\label{subfig:16325}
\includegraphics[scale=0.32,angle=270]{mater-band/16325}
}
\subfigure[NaNbSe$_{2}$ SG194 NoA=8 NoE=48]{
\label{subfig:26287}
\includegraphics[scale=0.32,angle=270]{mater-band/26287}
}
\subfigure[VAuS$_{2}$ SG194 NoA=8 NoE=56]{
\label{subfig:96089}
\includegraphics[scale=0.32,angle=270]{mater-band/96089}
}
\subfigure[LaGe SG63 NoA=8 NoE=60]{
\label{subfig:413736}
\includegraphics[scale=0.32,angle=270]{mater-band/413736}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[CrB SG141 NoA=8 NoE=36]{
\label{subfig:613476}
\includegraphics[scale=0.32,angle=270]{mater-band/613476}
}
\subfigure[SiPt$_{3}$ SG12 NoA=8 NoE=68]{
\label{subfig:246170}
\includegraphics[scale=0.32,angle=270]{mater-band/246170}
}
\subfigure[BW SG141 NoA=8 NoE=36]{
\label{subfig:424240}
\includegraphics[scale=0.32,angle=270]{mater-band/424240}
}
\subfigure[BMo SG141 NoA=8 NoE=36]{
\label{subfig:614793}
\includegraphics[scale=0.32,angle=270]{mater-band/614793}
}
\subfigure[InSe SG194 NoA=8 NoE=36]{
\label{subfig:185172}
\includegraphics[scale=0.32,angle=270]{mater-band/185172}
}
\subfigure[Si SG148 NoA=8 NoE=32]{
\label{subfig:109036}
\includegraphics[scale=0.32,angle=270]{mater-band/109036}
}
\subfigure[Cs$_{2}$Pd(IBr$_{2}$)$_{2}$ SG139 NoA=9 NoE=70]{
\label{subfig:240481}
\includegraphics[scale=0.32,angle=270]{mater-band/240481}
}
\subfigure[Ca$_{6}$Ge$_{2}$O SG225 NoA=9 NoE=74]{
\label{subfig:181078}
\includegraphics[scale=0.32,angle=270]{mater-band/181078}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Na(CuS)$_{4}$ SG164 NoA=9 NoE=69]{
\label{subfig:81306}
\includegraphics[scale=0.32,angle=270]{mater-band/81306}
}
\subfigure[CrSi$_{2}$ SG180 NoA=9 NoE=42]{
\label{subfig:626798}
\includegraphics[scale=0.32,angle=270]{mater-band/626798}
}
\subfigure[Li$_{5}$In$_{4}$ SG164 NoA=9 NoE=17]{
\label{subfig:639879}
\includegraphics[scale=0.32,angle=270]{mater-band/639879}
}
\subfigure[Nb$_{5}$Sb$_{4}$ SG87 NoA=9 NoE=75]{
\label{subfig:154596}
\includegraphics[scale=0.32,angle=270]{mater-band/154596}
}
\subfigure[CrSi$_{2}$ SG181 NoA=9 NoE=42]{
\label{subfig:96026}
\includegraphics[scale=0.32,angle=270]{mater-band/96026}
}
\subfigure[Si$_{2}$W SG180 NoA=9 NoE=42]{
\label{subfig:652549}
\includegraphics[scale=0.32,angle=270]{mater-band/652549}
}
\subfigure[Sr(RuO$_{3}$)$_{2}$ SG162 NoA=9 NoE=62]{
\label{subfig:248351}
\includegraphics[scale=0.32,angle=270]{mater-band/248351}
}
\subfigure[Si$_{2}$Mo SG180 NoA=9 NoE=42]{
\label{subfig:182116}
\includegraphics[scale=0.32,angle=270]{mater-band/182116}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[FePSe$_{3}$ SG148 NoA=10 NoE=62]{
\label{subfig:633091}
\includegraphics[scale=0.32,angle=270]{mater-band/633091}
}
\subfigure[Cs$_{2}$In$_{3}$ SG119 NoA=10 NoE=54]{
\label{subfig:102868}
\includegraphics[scale=0.32,angle=270]{mater-band/102868}
}
\subfigure[Sr(InP)$_{2}$ SG194 NoA=10 NoE=52]{
\label{subfig:260563}
\includegraphics[scale=0.32,angle=270]{mater-band/260563}
}
\subfigure[Rb$_{2}$As$_{3}$ SG69 NoA=10 NoE=66]{
\label{subfig:409381}
\includegraphics[scale=0.32,angle=270]{mater-band/409381}
}
\subfigure[NiPS$_{3}$ SG12 NoA=10 NoE=66]{
\label{subfig:602341}
\includegraphics[scale=0.32,angle=270]{mater-band/602341}
}
\subfigure[K$_{2}$Ga$_{3}$ SG139 NoA=10 NoE=54]{
\label{subfig:160496}
\includegraphics[scale=0.32,angle=270]{mater-band/160496}
}
\subfigure[Ca(GaP)$_{2}$ SG194 NoA=10 NoE=52]{
\label{subfig:422525}
\includegraphics[scale=0.32,angle=270]{mater-band/422525}
}
\subfigure[FePS$_{3}$ SG12 NoA=10 NoE=62]{
\label{subfig:61392}
\includegraphics[scale=0.32,angle=270]{mater-band/61392}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Ho$_{3}$Ni$_{2}$ SG12 NoA=10 NoE=94]{
\label{subfig:639449}
\includegraphics[scale=0.32,angle=270]{mater-band/639449}
}
\subfigure[Tb$_{3}$Ni$_{2}$ SG12 NoA=10 NoE=94]{
\label{subfig:646858}
\includegraphics[scale=0.32,angle=270]{mater-band/646858}
}
\subfigure[Dy$_{3}$Ni$_{2}$ SG12 NoA=10 NoE=94]{
\label{subfig:2334}
\includegraphics[scale=0.32,angle=270]{mater-band/2334}
}
\subfigure[Na$_{3}$Cl$_{2}$ SG83 NoA=10 NoE=34]{
\label{subfig:190543}
\includegraphics[scale=0.32,angle=270]{mater-band/190543}
}
\subfigure[Cs$_{2}$As$_{3}$ SG69 NoA=10 NoE=66]{
\label{subfig:409382}
\includegraphics[scale=0.32,angle=270]{mater-band/409382}
}
\subfigure[NiPSe$_{3}$ SG12 NoA=10 NoE=66]{
\label{subfig:646145}
\includegraphics[scale=0.32,angle=270]{mater-band/646145}
}
\subfigure[Y$_{4}$CI$_{5}$ SG12 NoA=10 NoE=83]{
\label{subfig:68014}
\includegraphics[scale=0.32,angle=270]{mater-band/68014}
}
\subfigure[Ba$_{3}$(LiAs)$_{4}$ SG71 NoA=11 NoE=54]{
\label{subfig:280027}
\includegraphics[scale=0.32,angle=270]{mater-band/280027}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Al$_{8}$Mo$_{3}$ SG12 NoA=11 NoE=42]{
\label{subfig:58001}
\includegraphics[scale=0.32,angle=270]{mater-band/58001}
}
\subfigure[Cu$_{2}$As$_{2}$O$_{7}$ SG12 NoA=11 NoE=74]{
\label{subfig:162061}
\includegraphics[scale=0.32,angle=270]{mater-band/162061}
}
\subfigure[Cu$_{2}$P$_{2}$O$_{7}$ SG12 NoA=11 NoE=74]{
\label{subfig:27436}
\includegraphics[scale=0.32,angle=270]{mater-band/27436}
}
\subfigure[Ir$_{3}$Se$_{8}$ SG148 NoA=11 NoE=75]{
\label{subfig:40823}
\includegraphics[scale=0.32,angle=270]{mater-band/40823}
}
\subfigure[CaGaGe SG194 NoA=12 NoE=68]{
\label{subfig:66002}
\includegraphics[scale=0.32,angle=270]{mater-band/66002}
}
\subfigure[NiAs$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:42569}
\includegraphics[scale=0.32,angle=270]{mater-band/42569}
}
\subfigure[ScCoSn SG62 NoA=12 NoE=64]{
\label{subfig:624977}
\includegraphics[scale=0.32,angle=270]{mater-band/624977}
}
\subfigure[TbGeIr SG62 NoA=12 NoE=88]{
\label{subfig:636739}
\includegraphics[scale=0.32,angle=270]{mater-band/636739}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[DyCoSn SG62 NoA=12 NoE=88]{
\label{subfig:54415}
\includegraphics[scale=0.32,angle=270]{mater-band/54415}
}
\subfigure[SiAs$_{2}$ SG205 NoA=12 NoE=56]{
\label{subfig:24801}
\includegraphics[scale=0.32,angle=270]{mater-band/24801}
}
\subfigure[LaAs$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:610769}
\includegraphics[scale=0.32,angle=270]{mater-band/610769}
}
\subfigure[RbNdTe$_{4}$ SG125 NoA=12 NoE=88]{
\label{subfig:412793}
\includegraphics[scale=0.32,angle=270]{mater-band/412793}
}
\subfigure[PrAs$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:611219}
\includegraphics[scale=0.32,angle=270]{mater-band/611219}
}
\subfigure[As$_{2}$Pd SG205 NoA=12 NoE=80]{
\label{subfig:43101}
\includegraphics[scale=0.32,angle=270]{mater-band/43101}
}
\subfigure[OsSe$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:24202}
\includegraphics[scale=0.32,angle=270]{mater-band/24202}
}
\subfigure[Te$_{2}$Os SG205 NoA=12 NoE=80]{
\label{subfig:300225}
\includegraphics[scale=0.32,angle=270]{mater-band/300225}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[RuSe$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:650607}
\includegraphics[scale=0.32,angle=270]{mater-band/650607}
}
\subfigure[OsS$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:24187}
\includegraphics[scale=0.32,angle=270]{mater-band/24187}
}
\subfigure[NdS$_{2}$ SG14 NoA=12 NoE=92]{
\label{subfig:419345}
\includegraphics[scale=0.32,angle=270]{mater-band/419345}
}
\subfigure[KNdTe$_{4}$ SG125 NoA=12 NoE=88]{
\label{subfig:412792}
\includegraphics[scale=0.32,angle=270]{mater-band/412792}
}
\subfigure[CuBIr SG43 NoA=12 NoE=92]{
\label{subfig:75029}
\includegraphics[scale=0.32,angle=270]{mater-band/75029}
}
\subfigure[ScCoSi SG62 NoA=12 NoE=64]{
\label{subfig:420415}
\includegraphics[scale=0.32,angle=270]{mater-band/420415}
}
\subfigure[Te$_{2}$Ru SG205 NoA=12 NoE=80]{
\label{subfig:65169}
\includegraphics[scale=0.32,angle=270]{mater-band/65169}
}
\subfigure[HoGeIr SG62 NoA=12 NoE=88]{
\label{subfig:88166}
\includegraphics[scale=0.32,angle=270]{mater-band/88166}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[LaTeAs SG62 NoA=12 NoE=88]{
\label{subfig:280231}
\includegraphics[scale=0.32,angle=270]{mater-band/280231}
}
\subfigure[CoAs$_{2}$ SG14 NoA=12 NoE=76]{
\label{subfig:610026}
\includegraphics[scale=0.32,angle=270]{mater-band/610026}
}
\subfigure[NdGeRh SG62 NoA=12 NoE=96]{
\label{subfig:82549}
\includegraphics[scale=0.32,angle=270]{mater-band/82549}
}
\subfigure[As$_{2}$Pt SG205 NoA=12 NoE=80]{
\label{subfig:24203}
\includegraphics[scale=0.32,angle=270]{mater-band/24203}
}
\subfigure[Bi$_{3}$Te$_{2}$S SG164 NoA=12 NoE=66]{
\label{subfig:107587}
\includegraphics[scale=0.32,angle=270]{mater-band/107587}
}
\subfigure[ZrFeSi SG62 NoA=12 NoE=96]{
\label{subfig:633674}
\includegraphics[scale=0.32,angle=270]{mater-band/633674}
}
\subfigure[ErGeIr SG62 NoA=12 NoE=88]{
\label{subfig:88167}
\includegraphics[scale=0.32,angle=270]{mater-band/88167}
}
\subfigure[FeSbTe SG14 NoA=12 NoE=76]{
\label{subfig:633405}
\includegraphics[scale=0.32,angle=270]{mater-band/633405}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[TbCoSi SG62 NoA=12 NoE=88]{
\label{subfig:88213}
\includegraphics[scale=0.32,angle=270]{mater-band/88213}
}
\subfigure[PrGeIr SG62 NoA=12 NoE=96]{
\label{subfig:636724}
\includegraphics[scale=0.32,angle=270]{mater-band/636724}
}
\subfigure[TbSiIr SG62 NoA=12 NoE=88]{
\label{subfig:93221}
\includegraphics[scale=0.32,angle=270]{mater-band/93221}
}
\subfigure[ScCoGe SG62 NoA=12 NoE=64]{
\label{subfig:428472}
\includegraphics[scale=0.32,angle=270]{mater-band/428472}
}
\subfigure[Bi$_{2}$Ir SG14 NoA=12 NoE=76]{
\label{subfig:424397}
\includegraphics[scale=0.32,angle=270]{mater-band/424397}
}
\subfigure[KPrTe$_{4}$ SG125 NoA=12 NoE=88]{
\label{subfig:391204}
\includegraphics[scale=0.32,angle=270]{mater-band/391204}
}
\subfigure[YbGaGe SG194 NoA=12 NoE=60]{
\label{subfig:152569}
\includegraphics[scale=0.32,angle=270]{mater-band/152569}
}
\subfigure[SiP$_{2}$ SG205 NoA=12 NoE=56]{
\label{subfig:30692}
\includegraphics[scale=0.32,angle=270]{mater-band/30692}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[ScGeRh SG62 NoA=12 NoE=64]{
\label{subfig:428475}
\includegraphics[scale=0.32,angle=270]{mater-band/428475}
}
\subfigure[Sb$_{2}$Pt SG205 NoA=12 NoE=80]{
\label{subfig:43105}
\includegraphics[scale=0.32,angle=270]{mater-band/43105}
}
\subfigure[TmGeIr SG62 NoA=12 NoE=88]{
\label{subfig:636748}
\includegraphics[scale=0.32,angle=270]{mater-band/636748}
}
\subfigure[ScSiRh SG62 NoA=12 NoE=64]{
\label{subfig:79596}
\includegraphics[scale=0.32,angle=270]{mater-band/79596}
}
\subfigure[Sb$_{2}$Rh SG14 NoA=12 NoE=76]{
\label{subfig:43501}
\includegraphics[scale=0.32,angle=270]{mater-band/43501}
}
\subfigure[DyCoSi SG62 NoA=12 NoE=88]{
\label{subfig:88272}
\includegraphics[scale=0.32,angle=270]{mater-band/88272}
}
\subfigure[RbPrTe$_{4}$ SG125 NoA=12 NoE=88]{
\label{subfig:412794}
\includegraphics[scale=0.32,angle=270]{mater-band/412794}
}
\subfigure[LuGeIr SG62 NoA=12 NoE=88]{
\label{subfig:412708}
\includegraphics[scale=0.32,angle=270]{mater-band/412708}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[As$_{2}$Rh SG14 NoA=12 NoE=76]{
\label{subfig:611271}
\includegraphics[scale=0.32,angle=270]{mater-band/611271}
}
\subfigure[Si SG63 NoA=12 NoE=48]{
\label{subfig:291479}
\includegraphics[scale=0.32,angle=270]{mater-band/291479}
}
\subfigure[CeZnGe SG194 NoA=12 NoE=108]{
\label{subfig:163343}
\includegraphics[scale=0.32,angle=270]{mater-band/163343}
}
\subfigure[SrNiGe SG62 NoA=12 NoE=96]{
\label{subfig:237303}
\includegraphics[scale=0.32,angle=270]{mater-band/237303}
}
\subfigure[NdAs$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:610996}
\includegraphics[scale=0.32,angle=270]{mater-band/610996}
}
\subfigure[CsIn$_{3}$ SG119 NoA=12 NoE=54]{
\label{subfig:102867}
\includegraphics[scale=0.32,angle=270]{mater-band/102867}
}
\subfigure[FeSe$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:633475}
\includegraphics[scale=0.32,angle=270]{mater-band/633475}
}
\subfigure[FeSbSe SG14 NoA=12 NoE=76]{
\label{subfig:633399}
\includegraphics[scale=0.32,angle=270]{mater-band/633399}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[FeAsSe SG14 NoA=12 NoE=76]{
\label{subfig:610526}
\includegraphics[scale=0.32,angle=270]{mater-band/610526}
}
\subfigure[PrP$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:647944}
\includegraphics[scale=0.32,angle=270]{mater-band/647944}
}
\subfigure[HoP$_{5}$ SG11 NoA=12 NoE=68]{
\label{subfig:409185}
\includegraphics[scale=0.32,angle=270]{mater-band/409185}
}
\subfigure[GdS$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:421335}
\includegraphics[scale=0.32,angle=270]{mater-band/421335}
}
\subfigure[CoP$_{2}$ SG14 NoA=12 NoE=76]{
\label{subfig:38316}
\includegraphics[scale=0.32,angle=270]{mater-band/38316}
}
\subfigure[CdSe$_{2}$ SG205 NoA=12 NoE=96]{
\label{subfig:620416}
\includegraphics[scale=0.32,angle=270]{mater-band/620416}
}
\subfigure[NdP$_{5}$ SG11 NoA=12 NoE=72]{
\label{subfig:358}
\includegraphics[scale=0.32,angle=270]{mater-band/358}
}
\subfigure[CuAsS SG62 NoA=12 NoE=88]{
\label{subfig:34450}
\includegraphics[scale=0.32,angle=270]{mater-band/34450}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[FePSe SG14 NoA=12 NoE=76]{
\label{subfig:633093}
\includegraphics[scale=0.32,angle=270]{mater-band/633093}
}
\subfigure[RhN$_{2}$ SG14 NoA=12 NoE=76]{
\label{subfig:160624}
\includegraphics[scale=0.32,angle=270]{mater-band/160624}
}
\subfigure[PdN$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:191245}
\includegraphics[scale=0.32,angle=270]{mater-band/191245}
}
\subfigure[CsGa$_{3}$ SG119 NoA=12 NoE=54]{
\label{subfig:102863}
\includegraphics[scale=0.32,angle=270]{mater-band/102863}
}
\subfigure[ReTeS SG216 NoA=12 NoE=76]{
\label{subfig:82721}
\includegraphics[scale=0.32,angle=270]{mater-band/82721}
}
\subfigure[HgO$_{2}$ SG61 NoA=12 NoE=96]{
\label{subfig:24774}
\includegraphics[scale=0.32,angle=270]{mater-band/24774}
}
\subfigure[NiP$_{2}$ SG205 NoA=12 NoE=80]{
\label{subfig:22221}
\includegraphics[scale=0.32,angle=270]{mater-band/22221}
}
\subfigure[PdSe$_{2}$ SG61 NoA=12 NoE=88]{
\label{subfig:648826}
\includegraphics[scale=0.32,angle=270]{mater-band/648826}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[LaZnSn SG194 NoA=12 NoE=108]{
\label{subfig:152623}
\includegraphics[scale=0.32,angle=270]{mater-band/152623}
}
\subfigure[SmP$_{5}$ SG11 NoA=12 NoE=72]{
\label{subfig:409183}
\includegraphics[scale=0.32,angle=270]{mater-band/409183}
}
\subfigure[SrGaSn SG194 NoA=12 NoE=68]{
\label{subfig:166387}
\includegraphics[scale=0.32,angle=270]{mater-band/166387}
}
\subfigure[FePS SG14 NoA=12 NoE=76]{
\label{subfig:633086}
\includegraphics[scale=0.32,angle=270]{mater-band/633086}
}
\subfigure[LaSe$_{2}$ SG14 NoA=12 NoE=92]{
\label{subfig:32530}
\includegraphics[scale=0.32,angle=270]{mater-band/32530}
}
\subfigure[TmP$_{5}$ SG11 NoA=12 NoE=68]{
\label{subfig:409186}
\includegraphics[scale=0.32,angle=270]{mater-band/409186}
}
\subfigure[BiOsSe SG14 NoA=12 NoE=76]{
\label{subfig:616892}
\includegraphics[scale=0.32,angle=270]{mater-band/616892}
}
\subfigure[YP$_{5}$ SG11 NoA=12 NoE=72]{
\label{subfig:409188}
\includegraphics[scale=0.32,angle=270]{mater-band/409188}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[TbS$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:422672}
\includegraphics[scale=0.32,angle=270]{mater-band/422672}
}
\subfigure[CoAsS SG14 NoA=12 NoE=80]{
\label{subfig:41858}
\includegraphics[scale=0.32,angle=270]{mater-band/41858}
}
\subfigure[DyP$_{5}$ SG11 NoA=12 NoE=68]{
\label{subfig:409184}
\includegraphics[scale=0.32,angle=270]{mater-band/409184}
}
\subfigure[PrP$_{5}$ SG11 NoA=12 NoE=72]{
\label{subfig:409182}
\includegraphics[scale=0.32,angle=270]{mater-band/409182}
}
\subfigure[ErS$_{2}$ SG14 NoA=12 NoE=84]{
\label{subfig:422673}
\includegraphics[scale=0.32,angle=270]{mater-band/422673}
}
\subfigure[KGa$_{3}$ SG119 NoA=12 NoE=54]{
\label{subfig:20664}
\includegraphics[scale=0.32,angle=270]{mater-band/20664}
}
\subfigure[LuP$_{5}$ SG11 NoA=12 NoE=68]{
\label{subfig:409187}
\includegraphics[scale=0.32,angle=270]{mater-band/409187}
}
\subfigure[IrN$_{2}$ SG14 NoA=12 NoE=76]{
\label{subfig:240755}
\includegraphics[scale=0.32,angle=270]{mater-band/240755}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[PrS$_{2}$ SG14 NoA=12 NoE=92]{
\label{subfig:92525}
\includegraphics[scale=0.32,angle=270]{mater-band/92525}
}
\subfigure[NdSe$_{2}$ SG14 NoA=12 NoE=92]{
\label{subfig:414619}
\includegraphics[scale=0.32,angle=270]{mater-band/414619}
}
\subfigure[PrSe$_{2}$ SG14 NoA=12 NoE=92]{
\label{subfig:413527}
\includegraphics[scale=0.32,angle=270]{mater-band/413527}
}
\subfigure[RbGa$_{3}$ SG119 NoA=12 NoE=54]{
\label{subfig:103943}
\includegraphics[scale=0.32,angle=270]{mater-band/103943}
}
\subfigure[YbB$_{12}$ SG225 NoA=13 NoE=44]{
\label{subfig:615734}
\includegraphics[scale=0.32,angle=270]{mater-band/615734}
}
\subfigure[Nb$_{7}$Co$_{6}$ SG166 NoA=13 NoE=131]{
\label{subfig:624284}
\includegraphics[scale=0.32,angle=270]{mater-band/624284}
}
\subfigure[Ba(P$_{2}$Au)$_{2}$ SG70 NoA=14 NoE=104]{
\label{subfig:425778}
\includegraphics[scale=0.32,angle=270]{mater-band/425778}
}
\subfigure[Sc$_{2}$Si$_{2}$Pt$_{3}$ SG55 NoA=14 NoE=88]{
\label{subfig:247425}
\includegraphics[scale=0.32,angle=270]{mater-band/247425}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Eu$_{2}$Zn$_{2}$P$_{3}$ SG12 NoA=14 NoE=114]{
\label{subfig:426082}
\includegraphics[scale=0.32,angle=270]{mater-band/426082}
}
\subfigure[Bi$_{4}$RuI$_{2}$ SG87 NoA=14 NoE=84]{
\label{subfig:406949}
\includegraphics[scale=0.32,angle=270]{mater-band/406949}
}
\subfigure[Sr$_{3}$(GeN)$_{2}$ SG11 NoA=14 NoE=96]{
\label{subfig:82533}
\includegraphics[scale=0.32,angle=270]{mater-band/82533}
}
\subfigure[Sr$_{2}$Zn$_{2}$As$_{3}$ SG12 NoA=14 NoE=118]{
\label{subfig:262413}
\includegraphics[scale=0.32,angle=270]{mater-band/262413}
}
\subfigure[Er$_{3}$Ni$_{2}$ SG148 NoA=15 NoE=141]{
\label{subfig:2150}
\includegraphics[scale=0.32,angle=270]{mater-band/2150}
}
\subfigure[Sb$_{2}$I$_{2}$F$_{11}$ SG5 NoA=15 NoE=101]{
\label{subfig:6031}
\includegraphics[scale=0.32,angle=270]{mater-band/6031}
}
\subfigure[Ho$_{3}$Ni$_{2}$ SG148 NoA=15 NoE=141]{
\label{subfig:639447}
\includegraphics[scale=0.32,angle=270]{mater-band/639447}
}
\subfigure[Ca$_{6}$Cr$_{2}$HN$_{6}$ SG148 NoA=15 NoE=103]{
\label{subfig:281462}
\includegraphics[scale=0.32,angle=270]{mater-band/281462}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Mn$_{4}$Al$_{11}$ SG2 NoA=15 NoE=61]{
\label{subfig:10509}
\includegraphics[scale=0.32,angle=270]{mater-band/10509}
}
\subfigure[Ba$_{4}$Fe$_{2}$S$_{4}$I$_{5}$ SG87 NoA=15 NoE=115]{
\label{subfig:173357}
\includegraphics[scale=0.32,angle=270]{mater-band/173357}
}
\subfigure[TcP$_{3}$ SG62 NoA=16 NoE=88]{
\label{subfig:35200}
\includegraphics[scale=0.32,angle=270]{mater-band/35200}
}
\subfigure[CoSb$_{3}$ SG204 NoA=16 NoE=96]{
\label{subfig:34048}
\includegraphics[scale=0.32,angle=270]{mater-band/34048}
}
\subfigure[Sb$_{3}$Ir SG204 NoA=16 NoE=96]{
\label{subfig:34050}
\includegraphics[scale=0.32,angle=270]{mater-band/34050}
}
\subfigure[Tl$_{2}$(CdSb)$_{3}$ SG12 NoA=16 NoE=114]{
\label{subfig:76500}
\includegraphics[scale=0.32,angle=270]{mater-band/76500}
}
\subfigure[LiSi SG88 NoA=16 NoE=40]{
\label{subfig:78364}
\includegraphics[scale=0.32,angle=270]{mater-band/78364}
}
\subfigure[ReP$_{3}$ SG62 NoA=16 NoE=88]{
\label{subfig:647985}
\includegraphics[scale=0.32,angle=270]{mater-band/647985}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[CdSb SG61 NoA=16 NoE=136]{
\label{subfig:52831}
\includegraphics[scale=0.32,angle=270]{mater-band/52831}
}
\subfigure[RhN$_{3}$ SG204 NoA=16 NoE=96]{
\label{subfig:162107}
\includegraphics[scale=0.32,angle=270]{mater-band/162107}
}
\subfigure[ZnAs SG61 NoA=16 NoE=136]{
\label{subfig:427612}
\includegraphics[scale=0.32,angle=270]{mater-band/427612}
}
\subfigure[SrP$_{3}$ SG12 NoA=16 NoE=100]{
\label{subfig:23628}
\includegraphics[scale=0.32,angle=270]{mater-band/23628}
}
\subfigure[In$_{3}$Ru SG136 NoA=16 NoE=68]{
\label{subfig:55514}
\includegraphics[scale=0.32,angle=270]{mater-band/55514}
}
\subfigure[NiP SG61 NoA=16 NoE=120]{
\label{subfig:27159}
\includegraphics[scale=0.32,angle=270]{mater-band/27159}
}
\subfigure[ZnSb SG61 NoA=16 NoE=136]{
\label{subfig:601137}
\includegraphics[scale=0.32,angle=270]{mater-band/601137}
}
\subfigure[Ga$_{3}$Ru SG136 NoA=16 NoE=68]{
\label{subfig:635229}
\includegraphics[scale=0.32,angle=270]{mater-band/635229}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[K$_{5}$Te$_{3}$ SG87 NoA=16 NoE=126]{
\label{subfig:66024}
\includegraphics[scale=0.32,angle=270]{mater-band/66024}
}
\subfigure[Ga$_{3}$Ir SG136 NoA=16 NoE=72]{
\label{subfig:634441}
\includegraphics[scale=0.32,angle=270]{mater-band/634441}
}
\subfigure[Ga$_{3}$Fe SG136 NoA=16 NoE=68]{
\label{subfig:103448}
\includegraphics[scale=0.32,angle=270]{mater-band/103448}
}
\subfigure[Mg$_{3}$In SG166 NoA=16 NoE=36]{
\label{subfig:51976}
\includegraphics[scale=0.32,angle=270]{mater-band/51976}
}
\subfigure[Ga$_{3}$Os SG136 NoA=16 NoE=68]{
\label{subfig:635023}
\includegraphics[scale=0.32,angle=270]{mater-band/635023}
}
\subfigure[SiPd$_{3}$ SG62 NoA=16 NoE=136]{
\label{subfig:648855}
\includegraphics[scale=0.32,angle=270]{mater-band/648855}
}
\subfigure[Hf$_{3}$Sb SG82 NoA=16 NoE=68]{
\label{subfig:638878}
\includegraphics[scale=0.32,angle=270]{mater-band/638878}
}
\subfigure[P$_{3}$Ir SG204 NoA=16 NoE=96]{
\label{subfig:640899}
\includegraphics[scale=0.32,angle=270]{mater-band/640899}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Li$_{3}$CaMnN$_{3}$ SG148 NoA=16 NoE=70]{
\label{subfig:408324}
\includegraphics[scale=0.32,angle=270]{mater-band/408324}
}
\subfigure[LiSi SG88 NoA=16 NoE=40]{
\label{subfig:96509}
\includegraphics[scale=0.32,angle=270]{mater-band/96509}
}
\subfigure[Ga$_{3}$Fe SG136 NoA=16 NoE=68]{
\label{subfig:103448}
\includegraphics[scale=0.32,angle=270]{mater-band/103448}
}
\subfigure[Al$_{2}$(FeSi)$_{3}$ SG2 NoA=16 NoE=84]{
\label{subfig:83664}
\includegraphics[scale=0.32,angle=270]{mater-band/83664}
}
\subfigure[La(FeAs$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:23080}
\includegraphics[scale=0.32,angle=270]{mater-band/23080}
}
\subfigure[Ce(As$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:610010}
\includegraphics[scale=0.32,angle=270]{mater-band/610010}
}
\subfigure[Pr(FeAs$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:610521}
\includegraphics[scale=0.32,angle=270]{mater-band/610521}
}
\subfigure[Ce(As$_{3}$Ru)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:610013}
\includegraphics[scale=0.32,angle=270]{mater-band/610013}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Nd(Sb$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:183088}
\includegraphics[scale=0.32,angle=270]{mater-band/183088}
}
\subfigure[Nd(FeSb$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:79927}
\includegraphics[scale=0.32,angle=270]{mater-band/79927}
}
\subfigure[Nd(As$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:611007}
\includegraphics[scale=0.32,angle=270]{mater-band/611007}
}
\subfigure[Pr(As$_{3}$Ru)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:611222}
\includegraphics[scale=0.32,angle=270]{mater-band/611222}
}
\subfigure[Nd(Sb$_{3}$Ru)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:645809}
\includegraphics[scale=0.32,angle=270]{mater-band/645809}
}
\subfigure[Ce(FeAs$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:610003}
\includegraphics[scale=0.32,angle=270]{mater-band/610003}
}
\subfigure[La(FeP$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:1286}
\includegraphics[scale=0.32,angle=270]{mater-band/1286}
}
\subfigure[La(P$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:641615}
\includegraphics[scale=0.32,angle=270]{mater-band/641615}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Nd(P$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:645670}
\includegraphics[scale=0.32,angle=270]{mater-band/645670}
}
\subfigure[Pr(Sb$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:155178}
\includegraphics[scale=0.32,angle=270]{mater-band/155178}
}
\subfigure[La(As$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:610776}
\includegraphics[scale=0.32,angle=270]{mater-band/610776}
}
\subfigure[Ce(Sb$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:621737}
\includegraphics[scale=0.32,angle=270]{mater-band/621737}
}
\subfigure[Pr(P$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:647712}
\includegraphics[scale=0.32,angle=270]{mater-band/647712}
}
\subfigure[Ce(Sb$_{3}$Ru)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:621988}
\includegraphics[scale=0.32,angle=270]{mater-band/621988}
}
\subfigure[La(Sb$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:183085}
\includegraphics[scale=0.32,angle=270]{mater-band/183085}
}
\subfigure[Ce(FeSb$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:621065}
\includegraphics[scale=0.32,angle=270]{mater-band/621065}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[La(FeSb$_{3}$)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:53490}
\includegraphics[scale=0.32,angle=270]{mater-band/53490}
}
\subfigure[Sm(Sb$_{3}$Os)$_{4}$ SG204 NoA=17 NoE=103]{
\label{subfig:647760}
\includegraphics[scale=0.32,angle=270]{mater-band/647760}
}
\subfigure[Ba$_{5}$Sb$_{4}$ SG64 NoA=18 NoE=140]{
\label{subfig:280022}
\includegraphics[scale=0.32,angle=270]{mater-band/280022}
}
\subfigure[Tm$_{5}$(ReO$_{6}$)$_{2}$ SG12 NoA=19 NoE=131]{
\label{subfig:280143}
\includegraphics[scale=0.32,angle=270]{mater-band/280143}
}
\subfigure[TiNb$_{3}$O$_{6}$ SG148 NoA=20 NoE=146]{
\label{subfig:280002}
\includegraphics[scale=0.32,angle=270]{mater-band/280002}
}
\subfigure[AlSiP$_{3}$ SG62 NoA=20 NoE=88]{
\label{subfig:10032}
\includegraphics[scale=0.32,angle=270]{mater-band/10032}
}
\subfigure[Bi$_{4}$I SG12 NoA=20 NoE=108]{
\label{subfig:246145}
\includegraphics[scale=0.32,angle=270]{mater-band/246145}
}
\subfigure[Sr(GaAs)$_{2}$ SG10 NoA=20 NoE=104]{
\label{subfig:422527}
\includegraphics[scale=0.32,angle=270]{mater-band/422527}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Nd$_{2}$SbO$_{2}$ SG59 NoA=20 NoE=156]{
\label{subfig:262307}
\includegraphics[scale=0.32,angle=270]{mater-band/262307}
}
\subfigure[BeSO$_{8}$ SG140 NoA=20 NoE=112]{
\label{subfig:36157}
\includegraphics[scale=0.32,angle=270]{mater-band/36157}
}
\subfigure[Mg$_{3}$Nb$_{6}$O$_{11}$ SG164 NoA=20 NoE=138]{
\label{subfig:200210}
\includegraphics[scale=0.32,angle=270]{mater-band/200210}
}
\subfigure[Nb$_{2}$F$_{5}$ SG229 NoA=21 NoE=171]{
\label{subfig:415950}
\includegraphics[scale=0.32,angle=270]{mater-band/415950}
}
\subfigure[Ba$_{5}$CrN$_{5}$ SG12 NoA=22 NoE=162]{
\label{subfig:82360}
\includegraphics[scale=0.32,angle=270]{mater-band/82360}
}
\subfigure[La$_{2}$Mo$_{2}$O$_{7}$ SG58 NoA=22 NoE=152]{
\label{subfig:202189}
\includegraphics[scale=0.32,angle=270]{mater-band/202189}
}
\subfigure[Sr(P$_{3}$Pt$_{2}$)$_{2}$ SG15 NoA=22 NoE=160]{
\label{subfig:62517}
\includegraphics[scale=0.32,angle=270]{mater-band/62517}
}
\subfigure[Nb$_{3}$Br$_{8}$ SG166 NoA=22 NoE=178]{
\label{subfig:25766}
\includegraphics[scale=0.32,angle=270]{mater-band/25766}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Ba(As$_{3}$Pt$_{2}$)$_{2}$ SG15 NoA=22 NoE=160]{
\label{subfig:62519}
\includegraphics[scale=0.32,angle=270]{mater-band/62519}
}
\subfigure[Sr(As$_{3}$Pt$_{2}$)$_{2}$ SG15 NoA=22 NoE=160]{
\label{subfig:62518}
\includegraphics[scale=0.32,angle=270]{mater-band/62518}
}
\subfigure[TiAs$_{2}$ SG58 NoA=24 NoE=112]{
\label{subfig:611500}
\includegraphics[scale=0.32,angle=270]{mater-band/611500}
}
\subfigure[LuCrB$_{4}$ SG55 NoA=24 NoE=108]{
\label{subfig:613517}
\includegraphics[scale=0.32,angle=270]{mater-band/613517}
}
\subfigure[LiGeTe$_{2}$ SG2 NoA=24 NoE=102]{
\label{subfig:35676}
\includegraphics[scale=0.32,angle=270]{mater-band/35676}
}
\subfigure[ErCrB$_{4}$ SG55 NoA=24 NoE=108]{
\label{subfig:613495}
\includegraphics[scale=0.32,angle=270]{mater-band/613495}
}
\subfigure[BaP$_{3}$Pt$_{2}$ SG14 NoA=24 NoE=180]{
\label{subfig:62520}
\includegraphics[scale=0.32,angle=270]{mater-band/62520}
}
\subfigure[YCrB$_{4}$ SG55 NoA=24 NoE=116]{
\label{subfig:16171}
\includegraphics[scale=0.32,angle=270]{mater-band/16171}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[TiCl$_{3}$ SG12 NoA=24 NoE=150]{
\label{subfig:39429}
\includegraphics[scale=0.32,angle=270]{mater-band/39429}
}
\subfigure[HoCrB$_{4}$ SG55 NoA=24 NoE=108]{
\label{subfig:613514}
\includegraphics[scale=0.32,angle=270]{mater-band/613514}
}
\subfigure[YB$_{4}$Mo SG55 NoA=24 NoE=116]{
\label{subfig:20081}
\includegraphics[scale=0.32,angle=270]{mater-band/20081}
}
\subfigure[CoGeTe SG61 NoA=24 NoE=152]{
\label{subfig:419780}
\includegraphics[scale=0.32,angle=270]{mater-band/419780}
}
\subfigure[NdPS SG62 NoA=24 NoE=176]{
\label{subfig:645690}
\includegraphics[scale=0.32,angle=270]{mater-band/645690}
}
\subfigure[GeTeRh SG61 NoA=24 NoE=152]{
\label{subfig:260373}
\includegraphics[scale=0.32,angle=270]{mater-band/260373}
}
\subfigure[ErPS SG62 NoA=24 NoE=160]{
\label{subfig:630913}
\includegraphics[scale=0.32,angle=270]{mater-band/630913}
}
\subfigure[YbNiB$_{4}$ SG55 NoA=24 NoE=120]{
\label{subfig:409820}
\includegraphics[scale=0.32,angle=270]{mater-band/409820}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[PrPS SG62 NoA=24 NoE=176]{
\label{subfig:647960}
\includegraphics[scale=0.32,angle=270]{mater-band/647960}
}
\subfigure[CeCrB$_{4}$ SG55 NoA=24 NoE=116]{
\label{subfig:612757}
\includegraphics[scale=0.32,angle=270]{mater-band/612757}
}
\subfigure[TbCrB$_{4}$ SG55 NoA=24 NoE=108]{
\label{subfig:613559}
\includegraphics[scale=0.32,angle=270]{mater-band/613559}
}
\subfigure[DyCrB$_{4}$ SG55 NoA=24 NoE=108]{
\label{subfig:658658}
\includegraphics[scale=0.32,angle=270]{mater-band/658658}
}
\subfigure[TmPS SG62 NoA=24 NoE=160]{
\label{subfig:648073}
\includegraphics[scale=0.32,angle=270]{mater-band/648073}
}
\subfigure[YPS SG62 NoA=24 NoE=176]{
\label{subfig:648080}
\includegraphics[scale=0.32,angle=270]{mater-band/648080}
}
\subfigure[KGaSb$_{4}$ SG62 NoA=24 NoE=128]{
\label{subfig:300158}
\includegraphics[scale=0.32,angle=270]{mater-band/300158}
}
\subfigure[HfSb$_{2}$ SG58 NoA=24 NoE=112]{
\label{subfig:638875}
\includegraphics[scale=0.32,angle=270]{mater-band/638875}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Y$_{4}$InIr SG216 NoA=24 NoE=224]{
\label{subfig:418567}
\includegraphics[scale=0.32,angle=270]{mater-band/418567}
}
\subfigure[ZrBi$_{2}$ SG58 NoA=24 NoE=176]{
\label{subfig:42880}
\includegraphics[scale=0.32,angle=270]{mater-band/42880}
}
\subfigure[Ho$_{4}$InIr SG216 NoA=24 NoE=192]{
\label{subfig:418270}
\includegraphics[scale=0.32,angle=270]{mater-band/418270}
}
\subfigure[Er$_{4}$InIr SG216 NoA=24 NoE=192]{
\label{subfig:418265}
\includegraphics[scale=0.32,angle=270]{mater-band/418265}
}
\subfigure[ZrSb$_{2}$ SG58 NoA=24 NoE=176]{
\label{subfig:66779}
\includegraphics[scale=0.32,angle=270]{mater-band/66779}
}
\subfigure[SmPS SG62 NoA=24 NoE=176]{
\label{subfig:648052}
\includegraphics[scale=0.32,angle=270]{mater-band/648052}
}
\subfigure[HfBi$_{2}$ SG58 NoA=24 NoE=112]{
\label{subfig:616683}
\includegraphics[scale=0.32,angle=270]{mater-band/616683}
}
\subfigure[Ba$_{2}$LiSi$_{3}$ SG70 NoA=24 NoE=132]{
\label{subfig:404707}
\includegraphics[scale=0.32,angle=270]{mater-band/404707}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Tm$_{4}$InRh SG216 NoA=24 NoE=192]{
\label{subfig:417519}
\includegraphics[scale=0.32,angle=270]{mater-band/417519}
}
\subfigure[Tb$_{4}$InRh SG216 NoA=24 NoE=192]{
\label{subfig:417518}
\includegraphics[scale=0.32,angle=270]{mater-band/417518}
}
\subfigure[Ba$_{2}$LiGe$_{3}$ SG70 NoA=24 NoE=132]{
\label{subfig:404705}
\includegraphics[scale=0.32,angle=270]{mater-band/404705}
}
\subfigure[Ho$_{4}$InRh SG216 NoA=24 NoE=192]{
\label{subfig:417517}
\includegraphics[scale=0.32,angle=270]{mater-band/417517}
}
\subfigure[Sr$_{2}$LiSi$_{3}$ SG70 NoA=24 NoE=132]{
\label{subfig:409295}
\includegraphics[scale=0.32,angle=270]{mater-band/409295}
}
\subfigure[KAlSb$_{4}$ SG62 NoA=24 NoE=128]{
\label{subfig:300157}
\includegraphics[scale=0.32,angle=270]{mater-band/300157}
}
\subfigure[FeS SG14 NoA=24 NoE=168]{
\label{subfig:89380}
\includegraphics[scale=0.32,angle=270]{mater-band/89380}
}
\subfigure[Ba$_{2}$Si$_{3}$Ag SG70 NoA=24 NoE=172]{
\label{subfig:410520}
\includegraphics[scale=0.32,angle=270]{mater-band/410520}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[KTl SG64 NoA=24 NoE=144]{
\label{subfig:262063}
\includegraphics[scale=0.32,angle=270]{mater-band/262063}
}
\subfigure[TbPS SG62 NoA=24 NoE=160]{
\label{subfig:648063}
\includegraphics[scale=0.32,angle=270]{mater-band/648063}
}
\subfigure[HoPS SG62 NoA=24 NoE=160]{
\label{subfig:639545}
\includegraphics[scale=0.32,angle=270]{mater-band/639545}
}
\subfigure[LaPS SG62 NoA=24 NoE=176]{
\label{subfig:641637}
\includegraphics[scale=0.32,angle=270]{mater-band/641637}
}
\subfigure[Ba$_{3}$Sb$_{2}$O SG55 NoA=24 NoE=184]{
\label{subfig:280592}
\includegraphics[scale=0.32,angle=270]{mater-band/280592}
}
\subfigure[Dy$_{4}$InRh SG216 NoA=24 NoE=192]{
\label{subfig:417514}
\includegraphics[scale=0.32,angle=270]{mater-band/417514}
}
\subfigure[DyPS SG62 NoA=24 NoE=160]{
\label{subfig:630062}
\includegraphics[scale=0.32,angle=270]{mater-band/630062}
}
\subfigure[Er$_{4}$InRh SG216 NoA=24 NoE=192]{
\label{subfig:417515}
\includegraphics[scale=0.32,angle=270]{mater-band/417515}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[SiSbPt SG61 NoA=24 NoE=152]{
\label{subfig:413194}
\includegraphics[scale=0.32,angle=270]{mater-band/413194}
}
\subfigure[Yb(Al$_{5}$Ru)$_{2}$ SG63 NoA=26 NoE=108]{
\label{subfig:186915}
\includegraphics[scale=0.32,angle=270]{mater-band/186915}
}
\subfigure[Ba$_{3}$(Si$_{2}$P$_{3}$)$_{2}$ SG11 NoA=26 NoE=152]{
\label{subfig:29261}
\includegraphics[scale=0.32,angle=270]{mater-band/29261}
}
\subfigure[Yb(Al$_{5}$Os)$_{2}$ SG63 NoA=26 NoE=108]{
\label{subfig:238040}
\includegraphics[scale=0.32,angle=270]{mater-band/238040}
}
\subfigure[Yb(Al$_{5}$Fe)$_{2}$ SG63 NoA=26 NoE=108]{
\label{subfig:151140}
\includegraphics[scale=0.32,angle=270]{mater-band/151140}
}
\subfigure[CuAgPO$_{4}$ SG14 NoA=28 NoE=204]{
\label{subfig:165596}
\includegraphics[scale=0.32,angle=270]{mater-band/165596}
}
\subfigure[La$_{3}$PI$_{3}$ SG214 NoA=28 NoE=236]{
\label{subfig:411801}
\includegraphics[scale=0.32,angle=270]{mater-band/411801}
}
\subfigure[Cs$_{3}$Zr$_{2}$I$_{9}$ SG194 NoA=28 NoE=228]{
\label{subfig:26565}
\includegraphics[scale=0.32,angle=270]{mater-band/26565}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Na$_{7}$Al$_{2}$Sb$_{5}$ SG11 NoA=28 NoE=76]{
\label{subfig:48168}
\includegraphics[scale=0.32,angle=270]{mater-band/48168}
}
\subfigure[La$_{3}$AsI$_{3}$ SG214 NoA=28 NoE=236]{
\label{subfig:411803}
\includegraphics[scale=0.32,angle=270]{mater-band/411803}
}
\subfigure[Sr$_{11}$(CdSb$_{2}$)$_{6}$ SG12 NoA=29 NoE=242]{
\label{subfig:413701}
\includegraphics[scale=0.32,angle=270]{mater-band/413701}
}
\subfigure[Ba$_{11}$(CdSb$_{2}$)$_{6}$ SG12 NoA=29 NoE=242]{
\label{subfig:418886}
\includegraphics[scale=0.32,angle=270]{mater-band/418886}
}
\subfigure[Nb$_{6}$Fe$_{16}$Si$_{7}$ SG225 NoA=29 NoE=222]{
\label{subfig:107097}
\includegraphics[scale=0.32,angle=270]{mater-band/107097}
}
\subfigure[Ta$_{6}$Fe$_{16}$Si$_{7}$ SG225 NoA=29 NoE=186]{
\label{subfig:107098}
\includegraphics[scale=0.32,angle=270]{mater-band/107098}
}
\subfigure[Mn$_{2}$P$_{12}$W SG15 NoA=30 NoE=160]{
\label{subfig:643287}
\includegraphics[scale=0.32,angle=270]{mater-band/643287}
}
\subfigure[Ba$_{4}$Li$_{2}$(CdAs$_{2}$)$_{3}$ SG63 NoA=30 NoE=216]{
\label{subfig:427778}
\includegraphics[scale=0.32,angle=270]{mater-band/427778}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Mn$_{2}$MoP$_{12}$ SG15 NoA=30 NoE=160]{
\label{subfig:68107}
\includegraphics[scale=0.32,angle=270]{mater-band/68107}
}
\subfigure[Sb$_{2}$MoSe SG14 NoA=32 NoE=176]{
\label{subfig:280615}
\includegraphics[scale=0.32,angle=270]{mater-band/280615}
}
\subfigure[Ta$_{3}$Ge SG86 NoA=32 NoE=152]{
\label{subfig:108870}
\includegraphics[scale=0.32,angle=270]{mater-band/108870}
}
\subfigure[SrSn$_{3}$Sb$_{4}$ SG62 NoA=32 NoE=168]{
\label{subfig:165617}
\includegraphics[scale=0.32,angle=270]{mater-band/165617}
}
\subfigure[RbNb$_{4}$Br$_{11}$ SG51 NoA=32 NoE=260]{
\label{subfig:380397}
\includegraphics[scale=0.32,angle=270]{mater-band/380397}
}
\subfigure[NaSn SG142 NoA=32 NoE=80]{
\label{subfig:409434}
\includegraphics[scale=0.32,angle=270]{mater-band/409434}
}
\subfigure[NaPb SG142 NoA=32 NoE=80]{
\label{subfig:105156}
\includegraphics[scale=0.32,angle=270]{mater-band/105156}
}
\subfigure[TlCu$_{5}$Se$_{3}$ SG136 NoA=36 NoE=304]{
\label{subfig:88202}
\includegraphics[scale=0.32,angle=270]{mater-band/88202}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Ta$_{4}$FeTe$_{4}$ SG55 NoA=36 NoE=208]{
\label{subfig:79796}
\includegraphics[scale=0.32,angle=270]{mater-band/79796}
}
\subfigure[K$_{6}$Na$_{14}$MgTl$_{18}$ SG200 NoA=39 NoE=124]{
\label{subfig:404695}
\includegraphics[scale=0.32,angle=270]{mater-band/404695}
}
\subfigure[K$_{6}$Na$_{14}$Tl$_{18}$Zn SG200 NoA=39 NoE=134]{
\label{subfig:236348}
\includegraphics[scale=0.32,angle=270]{mater-band/236348}
}
\subfigure[Ge$_{3}$Ru$_{2}$ SG60 NoA=40 NoE=224]{
\label{subfig:637743}
\includegraphics[scale=0.32,angle=270]{mater-band/637743}
}
\subfigure[Si$_{3}$Ru$_{2}$ SG60 NoA=40 NoE=224]{
\label{subfig:2344}
\includegraphics[scale=0.32,angle=270]{mater-band/2344}
}
\subfigure[Ba$_{11}$Sb$_{10}$ SG71 NoA=42 NoE=320]{
\label{subfig:413518}
\includegraphics[scale=0.32,angle=270]{mater-band/413518}
}
\subfigure[Ba$_{2}$(SnSb$_{2}$)$_{3}$ SG62 NoA=44 NoE=248]{
\label{subfig:82529}
\includegraphics[scale=0.32,angle=270]{mater-band/82529}
}
\subfigure[YB$_{7}$Mo$_{3}$ SG62 NoA=44 NoE=200]{
\label{subfig:39873}
\includegraphics[scale=0.32,angle=270]{mater-band/39873}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}

\begin{figure}[htp]
 \centering
\subfigure[Y$_{4}$BBr$_{6}$ SG15 NoA=44 NoE=356]{
\label{subfig:402661}
\includegraphics[scale=0.32,angle=270]{mater-band/402661}
}
\subfigure[Tb$_{4}$BBr$_{6}$ SG15 NoA=44 NoE=324]{
\label{subfig:410997}
\includegraphics[scale=0.32,angle=270]{mater-band/410997}
}
\subfigure[BaNb$_{8}$O$_{14}$ SG55 NoA=46 NoE=364]{
\label{subfig:79976}
\includegraphics[scale=0.32,angle=270]{mater-band/79976}
}
\subfigure[SrNb$_{8}$O$_{14}$ SG55 NoA=46 NoE=364]{
\label{subfig:202674}
\includegraphics[scale=0.32,angle=270]{mater-band/202674}
}
\subfigure[K(NaIn$_{3}$)$_{3}$ SG64 NoA=52 NoE=156]{
\label{subfig:165180}
\includegraphics[scale=0.32,angle=270]{mater-band/165180}
}
\subfigure[Nb$_{3}$Se$_{12}$I SG128 NoA=64 NoE=448]{
\label{subfig:72021}
\includegraphics[scale=0.32,angle=270]{mater-band/72021}
}
\subfigure[K$_{3}$Ga$_{13}$ SG63 NoA=64 NoE=264]{
\label{subfig:103709}
\includegraphics[scale=0.32,angle=270]{mater-band/103709}
}
\subfigure[Na$_{5}$Sn$_{13}$ SG63 NoA=144 NoE=456]{
\label{subfig:165613}
\includegraphics[scale=0.32,angle=270]{mater-band/165613}
}
\caption{\hyperref[tab:electride]{back to the table}}
\end{figure}



